Radio galaxies of the local universe: all-sky catalog, luminosity functions, and clustering

To understand the feedback of black holes on their environment or the acceleration of ultra-high energy cosmic rays in the present cosmic epoch, a systematic, all-sky inventory of radio galaxies in the local universe is needed. Here we present the first catalog of radio-emitting galaxies that meets this requirement. Our catalog allows the selection of volume-limited subsamples containing all low-power radio galaxies, similar to the prototypical low-power radio galaxies Cen A or M87, within some hundred Mpc. It is constructed by matching radio emission from the NVSS and SUMSS surveys to galaxies of the 2MASS Redshift Survey (2MRS) using an image-level algorithm that properly treats the extended structure of radio sources. The sample contains 575 radio-emitting galaxies with a flux greater than 213 mJy at 1.4 GHz. Over 30% of the galaxies in our catalog are not contained in existing large-area extra-galactic radio samples. We compute the optical and radio luminosity functions and the fraction of radio galaxies as a function of galaxy luminosity. We find that the galaxy density around radio galaxies is significantly higher than around non-radio galaxies of the same luminosity and morphology. This enhanced clustering suggests a causal relation between external galaxy properties, such as environment or merger history, and the formation of powerful jets in the present universe. Since the enhancement is observed with respect to galaxies of the same luminosity and Hubble type, it is not primarily driven by black hole mass. Our automated matching procedure is found to select radio-emitting galaxies with high efficiency (99%) and purity (91%), which is key for future processing of deeper, larger samples.

==> fulltab.tex <==
00031064$-$5444562 & $0.79429$ & $-54.74892$ & $0.03258$ & $140.2$ & $10.3$ & - & $1.5$ & $40.53$ & $0.84$ & j\\
00031298$-$3556132 & $0.80408$ & $-35.93708$ & $0.04976$ & $221.1$ & $10.9$ & $0.61$ & $1.1$ & $40.79$ & $2.3$ & j\\
00033830$+$5146404 & $0.90966$ & $51.77794$ & $0.04319$ & $194.7$ & $10.5$ & $0.49$ & - & $40.46$ & $3.5$ & u\\
00093552$-$3216365 & $2.39809$ & $-32.27686$ & $0.02546$ & $109.9$ & $9.7$ & $0.43$ & $0.56$ & $39.90$ & $2.4$ & j\\
00095929$-$5701148 & $2.49699$ & $-57.02082$ & $0.03157$ & $135.5$ & $10.0$ & - & $0.62$ & $40.10$ & $1.2$ & j\\
00112171$+$5231437 & $2.84041$ & $52.52882$ & $0.10432$ & $502.7$ & $11.7$ & $0.43$ & - & $41.22$ & $1.2$ & j\\
00145360$-$3911478 & $3.72334$ & $-39.19663$ & $0.00043$ & $2.0$ & $6.6$ & $0.22$ & - & $36.13$ & $7.3$ & g\\
00253146$-$3302458 & $6.38107$ & $-33.04613$ & $0.04970$ & $221.0$ & $11.4$ & $1.5$ & $2.3$ & $41.10$ & $2.0$ & j\\
00290096$-$0113420 & $7.25406$ & $-1.22829$ & $0.08281$ & $386.7$ & $11.4$ & $0.28$ & - & $40.81$ & $0.33$ & p\\
00345616$+$1027533 & $8.73405$ & $10.46487$ & $0.05690$ & $258.3$ & $11.5$ & $0.85$ & - & $40.94$ & $0.49$ & j\\
00375761$-$2504254 & $9.49014$ & $-25.07375$ & $0.06357$ & $288.3$ & $11.5$ & $0.22$ & - & $40.44$ & $1.9$ & j\\
00391857$+$0319528 & $9.82741$ & $3.33130$ & $0.01472$ & $60.0$ & $9.3$ & $1.3$ & - & $39.84$ & $2.6$ & j\\
00404885$-$5612504 & $10.20364$ & $-56.21407$ & $0.02720$ & $115.8$ & $10.0$ & - & $0.31$ & $39.67$ & $3.3$ & j\\
00473313$-$2517196 & $11.88806$ & $-25.28880$ & $0.00081$ & $3.5$ & $3.8$ & $5.6$ & - & $38.02$ & $14$ & g\\
00484711$+$3157249 & $12.19641$ & $31.95696$ & $0.01503$ & $62.3$ & $10.3$ & $0.29$ & - & $39.24$ & $0.30$ & p\\
00545264$-$0437033 & $13.71931$ & $-4.61759$ & $0.07154$ & $316.2$ & $11.7$ & $0.22$ & - & $40.53$ & $5.6$ & j\\
00560269$-$0120037 & $14.01125$ & $-1.33440$ & $0.04269$ & $190.2$ & $11.3$ & $1.2$ & - & $40.82$ & $5.2$ & j\\
00562558$-$0115449 & $14.10664$ & $-1.26248$ & $0.03823$ & $169.6$ & $10.6$ & $1.4$ & - & $40.78$ & $5.1$ & j\\
00573491$-$0123278 & $14.39547$ & $-1.39104$ & $0.04503$ & $201.2$ & $10.9$ & $5.4$ & - & $41.52$ & $1.5$ & j\\
00574891$+$3021083 & $14.45378$ & $30.35236$ & $0.01648$ & $69.7$ & $8.0$ & $6.6$ & - & $40.69$ & $8.2$ & j\\
00582263$+$2651586 & $14.59431$ & $26.86626$ & $0.04873$ & $220.0$ & $10.4$ & $1.8$ & - & $41.12$ & $5.3$ & j\\
00582305$-$6648461 & $14.59607$ & $-66.81281$ & $0.07431$ & $338.4$ & $11.4$ & - & $0.40$ & $40.72$ & $0.0$ & p\\
01014997$-$0252314 & $15.45820$ & $-2.87542$ & $0.07060$ & $324.6$ & $11.7$ & $0.25$ & - & $40.61$ & $6.8$ & j\\
01015074$-$0647594 & $15.46144$ & $-6.79981$ & $0.01997$ & $86.6$ & $9.3$ & $0.30$ & - & $39.53$ & $16$ & j\\
01072493$+$3224452 & $16.85396$ & $32.41256$ & $0.01701$ & $72.5$ & $8.6$ & $4.8$ & - & $40.59$ & $11$ & j\\
01074756$-$1730250 & $16.94818$ & $-17.50697$ & $0.02030$ & $87.4$ & $10.0$ & $0.25$ & - & $39.46$ & $0.26$ & p\\
01100320$+$1358417 & $17.51331$ & $13.97823$ & $0.05828$ & $265.0$ & $11.4$ & $0.24$ & - & $40.40$ & $0.92$ & p\\
01103850$+$1649348 & $17.66041$ & $16.82630$ & $0.06524$ & $299.1$ & $11.4$ & $0.30$ & - & $40.61$ & $1.4$ & j\\
01110909$-$1357397 & $17.78788$ & $-13.96103$ & $0.05164$ & $231.3$ & $10.7$ & $1.3$ & - & $41.03$ & $0.96$ & j\\
01125953$+$1529283 & $18.24813$ & $15.49125$ & $0.04385$ & $196.5$ & $10.8$ & $1.0$ & - & $40.79$ & $5.7$ & j\\
01193495$+$3210495 & $19.89573$ & $32.18051$ & $0.05971$ & $272.6$ & $11.3$ & $2.6$ & - & $41.47$ & $0.33$ & p\\
01254430$-$0122461 & $21.43460$ & $-1.37948$ & $0.01809$ & $76.2$ & $9.5$ & $0.54$ & - & $39.68$ & $4.0$ & j\\
01260057$-$0120424 & $21.50248$ & $-1.34514$ & $0.01824$ & $77.0$ & $8.5$ & $3.9$ & - & $40.55$ & $13$ & j\\
01265442$+$1912517 & $21.72676$ & $19.21446$ & $0.04268$ & $191.1$ & $10.9$ & $1.4$ & - & $40.89$ & $0.79$ & j\\
01313288$+$0033210 & $22.88709$ & $0.55589$ & $0.07924$ & $368.1$ & $11.7$ & $0.53$ & - & $41.04$ & $3.1$ & j\\
01335775$-$3629358 & $23.49057$ & $-36.49324$ & $0.03053$ & $131.9$ & $9.7$ & $5.1$ & $12$ & $41.38$ & $19$ & j\\
01341823$-$2925065 & $23.57598$ & $-29.41849$ & $0.00494$ & $20.6$ & $7.2$ & $0.22$ & - & $38.16$ & $3.4$ & g\\
01430234$+$1338444 & $25.75979$ & $13.64568$ & $0.00286$ & $12.4$ & $7.4$ & $0.39$ & - & $37.96$ & $2.7$ & g\\
01444275$+$4244154 & $26.17824$ & $42.73759$ & $0.05040$ & $228.1$ & $10.9$ & $0.29$ & - & $40.37$ & $2.3$ & j\\
01451214$-$5543394 & $26.30067$ & $-55.72767$ & $0.09009$ & $419.9$ & $11.6$ & - & $0.89$ & $41.24$ & $1.2$ & j\\
01532586$+$7115067 & $28.35774$ & $71.25183$ & $0.02281$ & $101.8$ & $9.8$ & $1.3$ & - & $40.31$ & $8.2$ & j\\
01562095$+$0537437 & $29.08735$ & $5.62887$ & $0.01855$ & $80.2$ & $8.4$ & $1.1$ & - & $40.02$ & $7.0$ & j\\
02093856$+$3547499 & $32.41074$ & $35.79723$ & $0.03773$ & $168.6$ & $9.4$ & $2.1$ & - & $40.96$ & $0.76$ & j\\
02105339$-$0633334 & $32.72250$ & $-6.55931$ & $0.04340$ & $192.6$ & $11.2$ & $0.62$ & - & $40.54$ & $1.1$ & j\\
02141794$+$5144520 & $33.57472$ & $51.74777$ & $0.04900$ & $221.4$ & $11.5$ & $0.45$ & - & $40.53$ & $4.8$ & j\\
02164508$-$4749086 & $34.18797$ & $-47.81908$ & $0.06427$ & $289.4$ & $11.0$ & - & $3.7$ & $41.54$ & $6.2$ & j\\
02195871$+$0155488 & $34.99468$ & $1.93024$ & $0.04103$ & $182.1$ & $10.7$ & $0.56$ & - & $40.45$ & $0.95$ & j\\
02202416$+$3659414 & $35.10069$ & $36.99483$ & $0.03680$ & $164.3$ & $10.7$ & $0.82$ & - & $40.53$ & $11$ & j\\
02221549$-$5106296 & $35.56444$ & $-51.10819$ & $0.04746$ & $208.5$ & $10.5$ & - & $0.71$ & $40.54$ & $8.1$ & j\\
02223290$+$4220539 & $35.63711$ & $42.34832$ & $0.00176$ & $9.3$ & $6.0$ & $0.70$ & - & $37.97$ & $4.8$ & g\\
02231298$+$4259162 & $35.80408$ & $42.98782$ & $0.02200$ & $97.9$ & $9.3$ & $6.2$ & - & $40.96$ & $8.4$ & j\\
02261765$-$1601094 & $36.57354$ & $-16.01924$ & $0.06636$ & $301.9$ & $11.5$ & $0.31$ & - & $40.64$ & $4.0$ & j\\
02283032$+$3821127 & $37.12638$ & $38.35346$ & $0.03280$ & $146.0$ & $11.5$ & $0.22$ & - & $39.85$ & $2.2$ & j\\
02293877$-$1702345 & $37.41164$ & $-17.04298$ & $0.05787$ & $260.3$ & $10.6$ & $0.24$ & - & $40.39$ & $1.3$ & p\\
02293889$+$2859154 & $37.41201$ & $28.98763$ & $0.04670$ & $209.8$ & $11.0$ & $0.60$ & - & $40.60$ & $1.1$ & j\\
02312619$-$1739129 & $37.85916$ & $-17.65366$ & $0.03294$ & $143.6$ & $10.8$ & $0.24$ & - & $39.88$ & $2.8$ & j\\
02341338$+$2918404 & $38.55573$ & $29.31127$ & $0.00515$ & $18.7$ & $7.9$ & $0.27$ & - & $38.16$ & $0.71$ & g\\
02351345$-$2936166 & $38.80609$ & $-29.60471$ & $0.05987$ & $269.1$ & $11.3$ & $0.25$ & - & $40.43$ & $2.8$ & j\\
02374181$+$0158309 & $39.42417$ & $1.97531$ & $0.02185$ & $94.1$ & $10.0$ & $0.23$ & - & $39.50$ & $12$ & j\\
02410480$-$0815209 & $40.26999$ & $-8.25583$ & $0.00530$ & $20.5$ & $7.5$ & $0.91$ & - & $38.77$ & $0.29$ & p\\
02410618$+$0844167 & $40.27572$ & $8.73801$ & $0.02080$ & $91.0$ & $9.7$ & $1.5$ & - & $40.27$ & $11$ & j\\
02424077$-$0000478 & $40.66988$ & $-0.01329$ & $0.00379$ & $15.5$ & $5.8$ & $4.8$ & - & $39.25$ & $0.27$ & g\\
02451349$+$1047230 & $41.30619$ & $10.78969$ & $0.07000$ & $321.5$ & $11.5$ & $0.42$ & - & $40.82$ & $1.5$ & j\\
02455992$-$0734431 & $41.49969$ & $-7.57864$ & $0.00479$ & $19.6$ & $8.0$ & $0.32$ & - & $38.27$ & $2.6$ & g\\
02460054$+$5115142 & $41.50220$ & $51.25399$ & $0.03479$ & $155.2$ & $10.6$ & $0.22$ & - & $39.91$ & $0.29$ & p\\
02461905$-$3016296 & $41.57941$ & $-30.27491$ & $0.00424$ & $18.6$ & $6.4$ & $0.41$ & $0.36$ & $38.34$ & $6.7$ & g\\
02493431$-$2030336 & $42.39305$ & $-20.50928$ & $0.08676$ & $404.6$ & $11.2$ & $1.0$ & - & $41.41$ & $7.2$ & j\\
02510087$+$4657175 & $42.75365$ & $46.95485$ & $0.02891$ & $128.5$ & $9.6$ & $0.77$ & - & $40.28$ & $18$ & j\\
02574155$+$0601371 & $44.42320$ & $6.02693$ & $0.02215$ & $96.6$ & $9.3$ & $6.0$ & - & $40.93$ & $11$ & j\\
02581124$-$5243419 & $44.54688$ & $-52.72832$ & $0.07274$ & $330.8$ & $11.2$ & - & $0.41$ & $40.70$ & $5.3$ & u\\
02592672$-$3940374 & $44.86129$ & $-39.67713$ & $0.06618$ & $299.0$ & $11.6$ & $0.98$ & $1.6$ & $41.19$ & $0.29$ & j\\
03002558$-$5150491 & $45.10657$ & $-51.84696$ & $0.07299$ & $332.1$ & $11.6$ & - & $0.68$ & $40.93$ & $2.0$ & j\\
03014235$+$3512203 & $45.42646$ & $35.20563$ & $0.01649$ & $74.4$ & $8.7$ & $1.8$ & - & $40.19$ & $0.29$ & p\\
03015146$+$3550283 & $45.46454$ & $35.84118$ & $0.04783$ & $215.1$ & $10.3$ & $0.76$ & - & $40.73$ & $2.1$ & j\\
03031501$+$1626188 & $45.81257$ & $16.43858$ & $0.03249$ & $143.4$ & $11.7$ & $3.1$ & - & $40.99$ & $2.5$ & j\\
03065268$-$1206234 & $46.71954$ & $-12.10655$ & $0.07876$ & $363.8$ & $11.4$ & $1.4$ & - & $41.44$ & $1.8$ & j\\
03082624$+$0406388 & $47.10933$ & $4.11083$ & $0.02865$ & $125.3$ & $9.1$ & $7.6$ & - & $41.26$ & $3.2$ & j\\
03101413$+$4249449 & $47.55898$ & $42.82915$ & $0.02890$ & $128.2$ & $11.7$ & $1.2$ & - & $40.48$ & $3.7$ & j\\
03143297$-$3407398 & $48.63732$ & $-34.12777$ & $0.06723$ & $304.4$ & $11.5$ & $0.47$ & $0.65$ & $40.83$ & $0.47$ & p\\
03163934$-$4351169 & $49.16389$ & $-43.85472$ & $0.06202$ & $278.2$ & $11.1$ & - & $2.0$ & $41.24$ & $0.99$ & p\\
03164302$+$4119291 & $49.17918$ & $41.32483$ & $0.01885$ & $84.0$ & $9.2$ & $0.54$ & - & $39.76$ & $4.5$ & j\\
03194823$+$4130420 & $49.95098$ & $41.51168$ & $0.01756$ & $78.7$ & $8.4$ & $23$ & - & $41.33$ & $0.27$ & p\\
03203116$+$4306517 & $50.12991$ & $43.11440$ & $0.05240$ & $236.9$ & $11.0$ & $0.48$ & - & $40.62$ & $0.68$ & p\\
03203810$+$4304447 & $50.15888$ & $43.07915$ & $0.05170$ & $233.5$ & $10.8$ & $0.79$ & - & $40.82$ & $1.8$ & j\\
03204016$+$2727485 & $50.16736$ & $27.46346$ & $0.06438$ & $294.2$ & $11.7$ & $0.44$ & - & $40.76$ & $3.4$ & j\\
03212595$+$1806093 & $50.35811$ & $18.10266$ & $0.06362$ & $279.9$ & $11.5$ & $0.28$ & - & $40.52$ & $9.4$ & j\\
03224178$-$3712295 & $50.67412$ & $-37.20820$ & $0.00587$ & $20.9$ & $5.7$ & $0.25$ & $1.7\times 10^{2}$ & $40.92$ & $61$ & j\\
03253395$-$3927270 & $51.39144$ & $-39.45745$ & $0.06516$ & $283.2$ & $11.6$ & $0.21$ & - & $40.42$ & $7.5$ & j\\
03262510$+$0940135 & $51.60463$ & $9.67041$ & $0.03742$ & $165.2$ & $11.2$ & $0.30$ & - & $40.09$ & $8.4$ & j\\
03263530$+$0911052 & $51.64718$ & $9.18472$ & $0.06388$ & $290.7$ & $11.3$ & $0.23$ & - & $40.47$ & $0.33$ & p\\
03275421$+$0233419 & $51.97586$ & $2.56167$ & $0.03022$ & $132.1$ & $10.7$ & $5.2$ & - & $41.14$ & $2.8$ & j\\
03292389$+$3947318 & $52.34954$ & $39.79221$ & $0.02444$ & $108.0$ & $9.9$ & $1.5$ & - & $40.41$ & $6.3$ & j\\
03312077$-$2606092 & $52.83659$ & $-26.10254$ & $0.06723$ & $304.8$ & $11.4$ & $0.48$ & - & $40.83$ & $1.3$ & u\\
03333645$-$3608263 & $53.40191$ & $-36.14066$ & $0.00555$ & $19.6$ & $6.6$ & $0.53$ & $0.64$ & $38.50$ & $8.0$ & g\\
03340335$-$3900360 & $53.51389$ & $-39.01004$ & $0.06231$ & $279.8$ & $11.7$ & $1.6$ & $2.9$ & $41.40$ & $5.5$ & j\\
03341837$+$3921243 & $53.57664$ & $39.35676$ & $0.02059$ & $91.0$ & $9.3$ & $0.96$ & - & $40.08$ & $1.6$ & j\\
03363741$-$3947383 & $54.15585$ & $-39.79397$ & $0.06732$ & $304.3$ & $11.6$ & $0.30$ & $0.46$ & $40.68$ & $1.4$ & u\\
03381409$+$1005038 & $54.55871$ & $10.08436$ & $0.03819$ & $168.6$ & $10.2$ & $0.42$ & - & $40.26$ & $2.0$ & j\\
03382908$-$3527026 & $54.62118$ & $-35.45074$ & $0.00475$ & $19.0$ & $6.4$ & $0.64$ & $0.96$ & $38.59$ & $4.4$ & j\\
03464851$+$6805459 & $56.70214$ & $68.09611$ & $0.00010$ & $3.8$ & $4.7$ & $2.4$ & - & $37.72$ & $20$ & g\\
03475994$+$4043586 & $56.99986$ & $40.73300$ & $0.03900$ & $173.8$ & $11.3$ & $0.97$ & - & $40.65$ & $0.66$ & j\\
03482073$+$7007583 & $57.08638$ & $70.13288$ & $0.00400$ & $17.1$ & $7.1$ & $0.46$ & - & $38.31$ & $2.1$ & g\\
03540284$-$0834301 & $58.51192$ & $-8.57499$ & $0.03298$ & $143.5$ & $11.0$ & $0.27$ & - & $39.92$ & $5.9$ & j\\
03543892$-$2030088 & $58.66220$ & $-20.50245$ & $0.00566$ & $23.5$ & $8.6$ & $0.24$ & - & $38.30$ & $0.26$ & p\\
03565430$+$0013313 & $59.22623$ & $0.22537$ & $0.04185$ & $184.7$ & $11.6$ & $0.55$ & - & $40.46$ & $3.1$ & j\\
03571349$+$3757160 & $59.30620$ & $37.95454$ & $0.05490$ & $248.3$ & $11.1$ & $0.26$ & - & $40.38$ & $3.4$ & j\\
03585442$+$1026033 & $59.72679$ & $10.43418$ & $0.03045$ & $133.2$ & $11.1$ & $11$ & - & $41.48$ & $4.0$ & j\\
04021299$+$1929075 & $60.55420$ & $19.48545$ & $0.05488$ & $247.2$ & $11.5$ & $0.78$ & - & $40.86$ & $1.7$ & j\\
04074251$-$2242549 & $61.92714$ & $-22.71531$ & $0.03237$ & $139.7$ & $10.9$ & $0.35$ & - & $40.02$ & $0.35$ & p\\
04082595$-$3100113 & $62.10813$ & $-31.00312$ & $0.05665$ & $252.5$ & $11.6$ & $0.89$ & - & $40.94$ & $3.0$ & j\\
04173578$-$6247012 & $64.39906$ & $-62.78367$ & $0.00435$ & $19.0$ & $8.0$ & - & $0.45$ & $38.26$ & $1.8$ & g\\
04200041$-$5456161 & $65.00175$ & $-54.93781$ & $0.00502$ & $20.4$ & $7.0$ & - & $0.30$ & $38.15$ & $2.0$ & g\\
04213310$+$1433544 & $65.38791$ & $14.56510$ & $0.05900$ & $266.6$ & $11.7$ & $0.27$ & - & $40.47$ & $1.1$ & j\\
04241857$-$2743437 & $66.07744$ & $-27.72886$ & $0.04971$ & $219.5$ & $11.6$ & $0.41$ & - & $40.47$ & $2.7$ & j\\
04290824$-$5349403 & $67.28423$ & $-53.82790$ & $0.03993$ & $172.4$ & $9.9$ & - & $8.1$ & $41.43$ & $8.6$ & j\\
04302197$-$6132001 & $67.59167$ & $-61.53347$ & $0.05550$ & $245.3$ & $11.2$ & - & $2.5$ & $41.22$ & $2.6$ & u\\
04304918$+$6450525 & $67.70494$ & $64.84792$ & $-0.00035$ & $2.5$ & $7.8$ & $0.36$ & - & $36.54$ & $3.5$ & g\\
04331106$+$0521151 & $68.29621$ & $5.35433$ & $0.03301$ & $144.1$ & $10.1$ & $4.1$ & - & $41.11$ & $5.3$ & j\\
04341042$-$1322119 & $68.54346$ & $-13.37000$ & $0.03478$ & $151.0$ & $11.3$ & $0.80$ & - & $40.44$ & $5.8$ & j\\
04363535$-$2226384 & $69.14732$ & $-22.44406$ & $0.06910$ & $313.6$ & $11.2$ & $1.1$ & - & $41.23$ & $6.7$ & j\\
04385802$+$0953336 & $69.74182$ & $9.89260$ & $0.02698$ & $117.1$ & $10.3$ & $0.47$ & - & $40.00$ & $8.2$ & j\\
04402651$-$4437590 & $70.11051$ & $-44.63307$ & $0.03333$ & $142.6$ & $10.5$ & - & $0.29$ & $39.83$ & $3.0$ & j\\
04454255$-$5914507 & $71.42730$ & $-59.24741$ & $0.00444$ & $20.1$ & $7.2$ & - & $0.29$ & $38.12$ & $0.70$ & g\\
04512060$-$1730121 & $72.83581$ & $-17.50340$ & $0.03157$ & $135.9$ & $10.3$ & $0.97$ & - & $40.43$ & $5.6$ & j\\
04531656$+$2552432 & $73.31905$ & $25.87864$ & $0.03399$ & $149.5$ & $10.0$ & $0.83$ & - & $40.45$ & $0.90$ & j\\
04541846$-$1855470 & $73.57689$ & $-18.92973$ & $0.03795$ & $164.9$ & $10.8$ & $0.36$ & - & $40.17$ & $0.62$ & j\\
04552373$-$2034159 & $73.84888$ & $-20.57109$ & $0.03536$ & $152.9$ & $10.3$ & $4.6$ & - & $41.21$ & $0.32$ & p\\
04594407$+$0519427 & $74.93363$ & $5.32857$ & $0.05379$ & $240.5$ & $11.6$ & $0.24$ & - & $40.32$ & $1.9$ & j\\
05030409$+$2300010 & $75.76700$ & $23.00033$ & $0.06399$ & $290.9$ & $11.7$ & $0.32$ & - & $40.62$ & $0.58$ & p\\
05045304$-$1014525 & $76.22105$ & $-10.24791$ & $0.04034$ & $176.3$ & $11.3$ & $1.5$ & - & $40.85$ & $0.31$ & p\\
05051445$-$3758507 & $76.31023$ & $-37.98075$ & $0.00392$ & $18.1$ & $7.1$ & $0.32$ & $0.36$ & $38.20$ & $4.0$ & g\\
05074234$-$3730469 & $76.92643$ & $-37.51305$ & $0.00323$ & $15.7$ & $6.7$ & $0.56$ & $0.81$ & $38.35$ & $2.8$ & g\\
05110479$-$1317309 & $77.77002$ & $-13.29187$ & $0.04305$ & $188.6$ & $10.8$ & $0.96$ & - & $40.71$ & $2.3$ & u\\
05143949$-$4903290 & $78.66451$ & $-49.05808$ & $0.09180$ & $427.8$ & $11.4$ & - & $1.1$ & $41.35$ & $0.90$ & j\\
05252717$-$3242157 & $81.36327$ & $-32.70434$ & $0.07681$ & $351.1$ & $11.3$ & $1.3$ & $1.8$ & $41.40$ & $3.8$ & j\\
05253863$-$3133103 & $81.41098$ & $-31.55281$ & $0.03432$ & $147.2$ & $11.2$ & $0.43$ & $0.60$ & $40.17$ & $0.48$ & j\\
05295057$+$2154537 & $82.46072$ & $21.91492$ & $0.05441$ & $244.1$ & $11.1$ & $0.44$ & - & $40.60$ & $3.4$ & j\\
05325578$+$5523356 & $83.23240$ & $55.39327$ & $0.04090$ & $182.3$ & $10.3$ & $0.22$ & - & $40.05$ & $10$ & j\\
05341281$-$5924194 & $83.55328$ & $-59.40533$ & $0.06559$ & $294.0$ & $11.7$ & - & $0.83$ & $40.91$ & $1.4$ & j\\
05444416$+$1648501 & $86.18403$ & $16.81393$ & $0.01951$ & $85.0$ & $9.8$ & $0.73$ & - & $39.91$ & $6.6$ & j\\
05462457$+$6321329 & $86.60249$ & $63.35910$ & $0.04900$ & $220.4$ & $10.8$ & $0.44$ & - & $40.51$ & $13$ & j\\
05481986$+$4144473 & $87.08269$ & $41.74647$ & $0.04457$ & $198.6$ & $10.9$ & $0.27$ & - & $40.21$ & $6.2$ & j\\
05482759$-$3258380 & $87.11501$ & $-32.97723$ & $0.03719$ & $160.0$ & $10.0$ & $1.3$ & $1.7$ & $40.71$ & $9.3$ & j\\
05492163$-$2520477 & $87.34015$ & $-25.34655$ & $0.03951$ & $171.0$ & $10.7$ & $0.25$ & - & $40.04$ & $2.7$ & j\\
05504985$-$3144266 & $87.70766$ & $-31.74072$ & $0.04003$ & $173.1$ & $11.2$ & $1.0$ & $1.8$ & $40.79$ & $6.2$ & p\\
05521140$-$0727222 & $88.04749$ & $-7.45620$ & $0.00804$ & $35.3$ & $8.1$ & $0.30$ & - & $38.75$ & $0.28$ & p\\
05545358$+$4626217 & $88.72334$ & $46.43934$ & $0.02048$ & $89.8$ & $9.2$ & $0.26$ & - & $39.50$ & $0.88$ & p\\
05571255$-$3728364 & $89.30229$ & $-37.47681$ & $0.04422$ & $192.2$ & $10.7$ & $0.30$ & $0.46$ & $40.28$ & $0.33$ & p\\
05581173$+$5328180 & $89.54904$ & $53.47165$ & $0.03496$ & $154.7$ & $11.2$ & $0.39$ & - & $40.15$ & $0.33$ & p\\
06020973$-$3956597 & $90.54052$ & $-39.94987$ & $0.04559$ & $198.5$ & $11.4$ & $0.40$ & $0.67$ & $40.47$ & $3.8$ & j\\
06065806$-$4929363 & $91.74198$ & $-49.49340$ & $0.05241$ & $230.3$ & $11.2$ & - & $1.5$ & $40.94$ & $1.5$ & j\\
06093663$+$0729211 & $92.40273$ & $7.48913$ & $0.05500$ & $245.5$ & $10.8$ & $0.27$ & - & $40.39$ & $4.7$ & j\\
06120351$-$3257472 & $93.01468$ & $-32.96313$ & $0.07791$ & $356.2$ & $11.4$ & $0.35$ & - & $40.83$ & $7.6$ & j\\
06153339$+$5158476 & $93.88911$ & $51.97989$ & $0.05013$ & $225.0$ & $10.7$ & $0.79$ & - & $40.78$ & $0.98$ & j\\
06153645$+$7102152 & $93.90173$ & $71.03753$ & $0.01351$ & $59.0$ & $9.0$ & $1.1$ & - & $39.77$ & $0.27$ & p\\
06162209$-$2122217 & $94.09206$ & $-21.37272$ & $0.00914$ & $37.4$ & $8.4$ & $0.39$ & - & $38.92$ & $3.6$ & g\\
06164203$+$6630240 & $94.17524$ & $66.50671$ & $0.01403$ & $61.1$ & $10.5$ & $0.29$ & - & $39.21$ & $0.31$ & p\\
06181305$-$4844580 & $94.55432$ & $-48.74951$ & $0.04682$ & $203.8$ & $10.9$ & - & $2.1$ & $41.00$ & $6.7$ & j\\
06183771$+$7821252 & $94.65713$ & $78.35702$ & $0.00298$ & $15.9$ & $7.1$ & $1.1$ & - & $38.62$ & $0.51$ & g\\
06200097$-$3711410 & $95.00407$ & $-37.19481$ & $0.03282$ & $139.7$ & $11.0$ & $2.9$ & $4.2$ & $40.96$ & $2.3$ & j\\
06214330$-$5241333 & $95.43043$ & $-52.69260$ & $0.05110$ & $223.9$ & $10.1$ & - & $4.8$ & $41.43$ & $5.0$ & j\\
06230765$-$6436211 & $95.78202$ & $-64.60579$ & $0.12889$ & $631.4$ & $11.5$ & - & $0.35$ & $41.19$ & $0.57$ & j\\
06233595$-$6434413 & $95.89975$ & $-64.57820$ & $0.04637$ & $201.3$ & $10.9$ & - & $0.38$ & $40.24$ & $5.1$ & j\\
06264958$-$5432340 & $96.70660$ & $-54.54287$ & $0.05198$ & $227.9$ & $11.1$ & - & $5.3$ & $41.49$ & $4.7$ & j\\
06265276$-$2437014 & $96.71985$ & $-24.61710$ & $0.02294$ & $94.8$ & $9.9$ & $0.26$ & - & $39.56$ & $4.2$ & j\\
06270669$-$3529152 & $96.77799$ & $-35.48760$ & $0.05485$ & $242.2$ & $10.7$ & $4.5$ & $6.3$ & $41.62$ & $2.4$ & j\\
06312271$+$2501067 & $97.84464$ & $25.01852$ & $0.08300$ & $385.5$ & $11.7$ & $1.1$ & - & $41.38$ & $1.8$ & j\\
06353594$+$2616376 & $98.89974$ & $26.27719$ & $0.04023$ & $177.0$ & $11.1$ & $0.93$ & - & $40.65$ & $1.2$ & j\\
06442508$-$4343484 & $101.10458$ & $-43.73016$ & $0.06152$ & $273.9$ & $11.2$ & - & $3.1$ & $41.42$ & $7.8$ & j\\
06502151$-$5549325 & $102.58959$ & $-55.82574$ & $0.04972$ & $217.1$ & $10.6$ & - & $1.9$ & $40.99$ & $5.7$ & j\\
06503056$+$2833345 & $102.62732$ & $28.55956$ & $0.06366$ & $288.4$ & $11.5$ & $0.46$ & - & $40.76$ & $6.9$ & j\\
06505914$+$1518493 & $102.74651$ & $15.31376$ & $0.05646$ & $252.6$ & $11.8$ & $0.85$ & - & $40.92$ & $1.1$ & j\\
06521236$+$7425372 & $103.05146$ & $74.42698$ & $0.01881$ & $82.7$ & $9.6$ & $0.27$ & - & $39.45$ & $0.33$ & p\\
06551006$+$4100097 & $103.79185$ & $41.00279$ & $0.02156$ & $93.6$ & $10.5$ & $0.23$ & - & $39.48$ & $0.28$ & p\\
06561069$+$4237023 & $104.04447$ & $42.61739$ & $0.05900$ & $266.6$ & $11.3$ & $0.93$ & - & $41.00$ & $0.51$ & j\\
07012902$+$2313260 & $105.37099$ & $23.22384$ & $0.09196$ & $431.7$ & $11.7$ & $0.98$ & - & $41.44$ & $5.6$ & j\\
07024038$-$2841501 & $105.66829$ & $-28.69725$ & $0.00729$ & $31.8$ & $8.0$ & $0.25$ & - & $38.59$ & $0.69$ & p\\
07042876$+$1835222 & $106.11981$ & $18.58949$ & $0.02604$ & $111.9$ & $10.3$ & $0.25$ & - & $39.67$ & $0.30$ & p\\
07074155$+$3503309 & $106.92321$ & $35.05860$ & $0.07850$ & $362.8$ & $11.6$ & $0.55$ & - & $41.04$ & $1.8$ & j\\
07090797$+$4836561 & $107.28328$ & $48.61554$ & $0.01933$ & $84.8$ & $9.4$ & $0.75$ & - & $39.91$ & $4.3$ & j\\
07135663$-$3501260 & $108.48600$ & $-35.02396$ & $0.04418$ & $191.4$ & $10.9$ & $0.34$ & $0.43$ & $40.28$ & $0.39$ & p\\
07163708$+$3642186 & $109.15459$ & $36.70517$ & $0.07027$ & $321.4$ & $11.3$ & $0.29$ & - & $40.66$ & $0.33$ & p\\
07164122$+$5323091 & $109.17177$ & $53.38594$ & $0.06361$ & $289.6$ & $10.5$ & $1.5$ & - & $41.28$ & $0.57$ & j\\
07170806$-$3621591 & $109.28367$ & $-36.36634$ & $0.03136$ & $132.6$ & $10.4$ & $2.5$ & $3.6$ & $40.85$ & $5.4$ & j\\
07171670$+$4308491 & $109.31954$ & $43.14693$ & $0.05660$ & $254.9$ & $11.0$ & $0.25$ & - & $40.39$ & $4.5$ & j\\
07172666$+$4405020 & $109.36107$ & $44.08398$ & $0.06520$ & $296.8$ & $11.5$ & $0.23$ & - & $40.48$ & $2.5$ & p\\
07175757$+$0941218 & $109.48984$ & $9.68934$ & $0.02862$ & $122.7$ & $10.9$ & $0.32$ & - & $39.86$ & $0.29$ & p\\
07181457$-$4711322 & $109.56081$ & $-47.19231$ & $0.04231$ & $182.4$ & $10.4$ & - & $0.91$ & $40.53$ & $4.3$ & j\\
07193787$+$5526064 & $109.90782$ & $55.43514$ & $0.06562$ & $299.6$ & $11.5$ & $0.33$ & - & $40.66$ & $1.1$ & j\\
07204757$-$3407058 & $110.19823$ & $-34.11834$ & $0.02835$ & $119.2$ & $10.1$ & $2.5$ & $3.1$ & $40.73$ & $1.7$ & j\\
07271448$+$8545162 & $111.80984$ & $85.75455$ & $0.00806$ & $38.0$ & $9.2$ & $0.29$ & - & $38.80$ & $3.9$ & g\\
07280854$-$3641594 & $112.03571$ & $-36.69991$ & $0.07091$ & $320.1$ & $11.5$ & $0.41$ & - & $40.80$ & $2.9$ & j\\
07331844$-$3654533 & $113.32696$ & $-36.91481$ & $0.02353$ & $97.5$ & $10.5$ & $0.20$ & $0.42$ & $39.65$ & $14$ & j\\
07332987$+$5742023 & $113.37456$ & $57.70060$ & $0.04172$ & $185.4$ & $11.3$ & $0.31$ & - & $40.20$ & $4.0$ & j\\
07373010$+$5941031 & $114.37540$ & $59.68421$ & $0.04054$ & $180.1$ & $10.6$ & $0.56$ & - & $40.44$ & $0.29$ & p\\
07483682$+$5548591 & $117.15347$ & $55.81637$ & $0.03566$ & $157.4$ & $10.9$ & $2.2$ & - & $40.92$ & $25$ & j\\
07524421$+$4556576 & $118.18421$ & $45.94932$ & $0.05169$ & $231.4$ & $11.5$ & $0.62$ & - & $40.70$ & $3.0$ & j\\
07545738$-$0222120 & $118.73908$ & $-2.37003$ & $0.08849$ & $411.2$ & $11.4$ & $0.70$ & - & $41.26$ & $3.9$ & u\\
07582810$+$3747121 & $119.61712$ & $37.78666$ & $0.04082$ & $179.8$ & $10.1$ & $2.7$ & - & $41.13$ & $1.9$ & j\\
07583734$+$0801468 & $119.65563$ & $8.02968$ & $0.03188$ & $136.9$ & $9.7$ & $0.54$ & - & $40.18$ & $1.1$ & j\\
08162288$-$7039398 & $124.09518$ & $-70.66105$ & $0.06978$ & $313.9$ & $11.0$ & - & $1.9$ & $41.33$ & $4.0$ & j\\
08173619$+$5957137 & $124.40091$ & $59.95378$ & $0.02859$ & $125.5$ & $10.3$ & $0.46$ & - & $40.05$ & $2.4$ & j\\
08180059$-$1613599 & $124.50249$ & $-16.23335$ & $0.05047$ & $221.2$ & $10.6$ & $0.45$ & - & $40.53$ & $0.29$ & p\\
08205880$-$5705337 & $125.24494$ & $-57.09267$ & $0.06024$ & $267.0$ & $11.1$ & - & $2.4$ & $41.28$ & $0.75$ & j\\
08353408$-$0151002 & $128.89197$ & $-1.85010$ & $0.03119$ & $132.8$ & $9.8$ & $0.94$ & - & $40.40$ & $6.5$ & j\\
08391582$+$2850389 & $129.81595$ & $28.84413$ & $0.07896$ & $364.0$ & $11.1$ & $0.92$ & - & $41.27$ & $5.7$ & j\\
08445266$-$1000590 & $131.21948$ & $-10.01641$ & $0.04287$ & $185.8$ & $11.3$ & $0.31$ & - & $40.21$ & $1.1$ & j\\
08450824$-$3347411 & $131.28436$ & $-33.79476$ & $0.00701$ & $30.0$ & $6.8$ & $2.6$ & $2.9$ & $39.55$ & $16$ & j\\
08471978$-$3320011 & $131.83234$ & $-33.33357$ & $0.03829$ & $163.6$ & $10.5$ & $0.32$ & - & $40.12$ & $5.8$ & j\\
08475313$+$5352344 & $131.97136$ & $53.87619$ & $0.04549$ & $202.4$ & $10.6$ & $1.5$ & - & $40.98$ & $0.51$ & p\\
08475906$+$3147083 & $131.99605$ & $31.78565$ & $0.06730$ & $305.7$ & $10.8$ & $1.6$ & - & $41.36$ & $3.9$ & j\\
08531896$+$6828187 & $133.32887$ & $68.47191$ & $0.04026$ & $179.1$ & $10.5$ & $0.30$ & - & $40.16$ & $1.6$ & j\\
09001815$+$0745350 & $135.07565$ & $7.75982$ & $0.06055$ & $270.7$ & $11.3$ & $0.24$ & - & $40.43$ & $4.4$ & j\\
09045929$-$1227444 & $136.24699$ & $-12.46241$ & $0.05604$ & $247.7$ & $11.1$ & $0.25$ & - & $40.37$ & $1.7$ & j\\
09074701$-$3535234 & $136.94585$ & $-35.58986$ & $0.03741$ & $159.4$ & $10.9$ & $1.6$ & $1.5$ & $40.79$ & $8.3$ & u\\
09080217$-$0959378 & $137.00914$ & $-9.99376$ & $0.05501$ & $235.5$ & $11.5$ & $0.64$ & - & $40.73$ & $7.9$ & j\\
09092633$-$0922471 & $137.35973$ & $-9.37983$ & $0.05852$ & $259.8$ & $11.4$ & $0.38$ & - & $40.59$ & $1.8$ & j\\
09101737$-$0937068 & $137.57236$ & $-9.61855$ & $0.05528$ & $244.2$ & $11.2$ & $0.46$ & - & $40.62$ & $4.1$ & j\\
09135500$-$1433516 & $138.47917$ & $-14.56429$ & $0.05510$ & $243.0$ & $11.3$ & $0.61$ & - & $40.74$ & $8.1$ & u\\
09180565$-$1205439 & $139.52356$ & $-12.09552$ & $0.05488$ & $242.1$ & $11.1$ & $41$ & - & $42.56$ & $1.0$ & j\\
09275281$+$2959085 & $141.97008$ & $29.98573$ & $0.02666$ & $114.5$ & $10.2$ & $0.40$ & - & $39.90$ & $25$ & j\\
09321011$+$2130029 & $143.04213$ & $21.50083$ & $0.00185$ & $10.4$ & $6.1$ & $0.44$ & - & $37.86$ & $2.0$ & g\\
09325289$+$6737026 & $143.22049$ & $67.61740$ & $0.02282$ & $100.1$ & $9.5$ & $0.24$ & - & $39.56$ & $1.7$ & j\\
09340714$-$3728078 & $143.52959$ & $-37.46885$ & $0.06294$ & $280.0$ & $11.3$ & $1.0$ & $1.4$ & $41.10$ & $2.3$ & j\\
09383601$-$0420061 & $144.65005$ & $-4.33509$ & $0.06968$ & $314.6$ & $11.3$ & $0.61$ & - & $40.96$ & $5.3$ & j\\
09395923$-$3307068 & $144.99686$ & $-33.11855$ & $0.04209$ & $180.9$ & $11.1$ & $0.39$ & $0.59$ & $40.33$ & $0.31$ & p\\
09422410$-$3044101 & $145.60036$ & $-30.73615$ & $0.03863$ & $165.0$ & $10.8$ & $0.35$ & $0.40$ & $40.17$ & $2.9$ & j\\
09453879$-$3111279 & $146.41164$ & $-31.19109$ & $0.00363$ & $12.5$ & $6.6$ & $0.22$ & $0.42$ & $37.87$ & $11$ & g\\
09454204$-$1419348 & $146.42519$ & $-14.32636$ & $0.00778$ & $34.9$ & $8.7$ & $0.23$ & - & $38.62$ & $0.32$ & p\\
09475094$-$3715272 & $146.96227$ & $-37.25753$ & $0.04125$ & $176.9$ & $11.3$ & $0.67$ & $0.97$ & $40.53$ & $2.2$ & j\\
09555243$+$6940469 & $148.96846$ & $69.67970$ & $0.00068$ & $3.7$ & $4.6$ & $6.4$ & - & $38.12$ & $1.0$ & g\\
09582458$-$2655356 & $149.60246$ & $-26.92660$ & $0.00865$ & $38.7$ & $7.9$ & $0.32$ & - & $38.86$ & $3.4$ & j\\
09592102$+$0117518 & $149.83752$ & $1.29786$ & $0.09760$ & $458.7$ & $11.6$ & $0.51$ & - & $41.21$ & $1.3$ & j\\
10002708$-$0754140 & $150.11287$ & $-7.90385$ & $0.03358$ & $142.9$ & $10.8$ & $0.27$ & - & $39.92$ & $2.6$ & j\\
10004083$-$3139519 & $150.17017$ & $-31.66449$ & $0.00861$ & $38.6$ & $8.2$ & $0.53$ & $0.72$ & $39.08$ & $0.31$ & j\\
10015792$+$5540480 & $150.49135$ & $55.68000$ & $0.00372$ & $19.6$ & $7.3$ & $0.87$ & - & $38.70$ & $2.2$ & g\\
10045181$+$5434046 & $151.21597$ & $54.56789$ & $0.04700$ & $209.4$ & $11.0$ & $0.23$ & - & $40.18$ & $17$ & j\\
10065190$+$1422247 & $151.71620$ & $14.37357$ & $0.02944$ & $125.6$ & $9.7$ & $0.76$ & - & $40.26$ & $5.2$ & j\\
10083368$-$0428393 & $152.14035$ & $-4.47767$ & $0.05090$ & $223.4$ & $11.4$ & $0.25$ & - & $40.28$ & $0.32$ & p\\
10275128$-$4354135 & $156.96364$ & $-43.90382$ & $0.00946$ & $40.6$ & $8.1$ & - & $1.1$ & $39.30$ & $0.0$ & p\\
10301064$-$0309488 & $157.54439$ & $-3.16363$ & $0.03797$ & $163.1$ & $10.0$ & $0.37$ & - & $40.17$ & $10$ & j\\
10325883$+$5644538 & $158.24522$ & $56.74823$ & $0.04484$ & $199.4$ & $10.6$ & $0.52$ & - & $40.49$ & $12$ & j\\
10360578$+$0006068 & $159.02408$ & $0.10190$ & $0.09683$ & $454.5$ & $11.7$ & $0.54$ & - & $41.23$ & $2.5$ & j\\
10393872$+$0510326 & $159.91142$ & $5.17568$ & $0.06790$ & $306.2$ & $11.5$ & $0.46$ & - & $40.82$ & $2.4$ & j\\
10431869$+$3131058 & $160.82779$ & $31.51835$ & $0.03562$ & $154.8$ & $11.3$ & $0.75$ & - & $40.44$ & $0.37$ & p\\
10460990$-$2921094 & $161.54134$ & $-29.35268$ & $0.05974$ & $264.5$ & $11.3$ & $0.59$ & - & $40.80$ & $4.2$ & j\\
10461032$+$7321108 & $161.54320$ & $73.35307$ & $0.02100$ & $92.4$ & $9.7$ & $0.70$ & - & $39.96$ & $1.1$ & j\\
10483217$-$4251276 & $162.13397$ & $-42.85773$ & $0.05680$ & $250.0$ & $11.7$ & - & $0.32$ & $40.35$ & $0.54$ & p\\
10492114$-$0040049 & $162.33807$ & $-0.66805$ & $0.03870$ & $166.6$ & $10.7$ & $0.26$ & - & $40.05$ & $0.72$ & j\\
10514731$+$5523087 & $162.94733$ & $55.38571$ & $0.07392$ & $340.3$ & $11.7$ & $0.53$ & - & $40.97$ & $3.6$ & j\\
11031119$+$2758207 & $165.79671$ & $27.97250$ & $0.00509$ & $24.3$ & $8.3$ & $0.27$ & - & $38.39$ & $0.38$ & p\\
11032753$-$4657471 & $165.86469$ & $-46.96302$ & $0.04920$ & $213.8$ & $11.5$ & - & $0.78$ & $40.60$ & $9.9$ & j\\
11042732$+$3812320 & $166.11382$ & $38.20885$ & $0.03002$ & $130.0$ & $10.1$ & $0.88$ & - & $40.35$ & $2.2$ & j\\
11052280$+$3009411 & $166.34505$ & $30.16148$ & $0.07166$ & $326.8$ & $11.5$ & $0.41$ & - & $40.82$ & $1.6$ & j\\
11054859$-$0002092 & $166.45247$ & $-0.03590$ & $0.00267$ & $12.7$ & $5.8$ & $0.38$ & - & $37.97$ & $4.2$ & g\\
11082650$-$1015216 & $167.11047$ & $-10.25604$ & $0.02730$ & $114.5$ & $9.7$ & $0.32$ & - & $39.81$ & $0.26$ & p\\
11095773$-$3732216 & $167.49054$ & $-37.53934$ & $0.01017$ & $44.0$ & $7.3$ & $0.67$ & $0.57$ & $39.30$ & $12$ & j\\
11113096$+$5540268 & $167.87903$ & $55.67412$ & $0.00233$ & $13.6$ & $7.1$ & $0.28$ & - & $37.90$ & $5.5$ & g\\
11125076$-$1219212 & $168.21149$ & $-12.32253$ & $0.06569$ & $294.3$ & $11.3$ & $0.39$ & - & $40.71$ & $5.2$ & j\\
11163458$+$2915166 & $169.14418$ & $29.25470$ & $0.04782$ & $211.2$ & $11.6$ & $1.9$ & - & $41.12$ & $1.1$ & j\\
11185938$+$2754070 & $169.74739$ & $27.90195$ & $0.06718$ & $304.4$ & $11.3$ & $0.52$ & - & $40.87$ & $3.0$ & j\\
11194398$+$1357503 & $169.93318$ & $13.96395$ & $0.06880$ & $311.4$ & $11.6$ & $0.29$ & - & $40.63$ & $5.5$ & j\\
11201502$+$1259286 & $170.06261$ & $12.99129$ & $0.00243$ & $10.1$ & $5.9$ & $0.45$ & - & $37.85$ & $3.4$ & g\\
11201701$+$1335221 & $170.07091$ & $13.58949$ & $0.00275$ & $13.7$ & $6.2$ & $0.34$ & - & $37.98$ & $3.5$ & g\\
11255292$-$3523402 & $171.47058$ & $-35.39457$ & $0.03375$ & $142.6$ & $9.8$ & $2.6$ & $3.7$ & $40.93$ & $3.0$ & j\\
11282461$-$1122184 & $172.10262$ & $-11.37174$ & $0.07687$ & $350.1$ & $11.5$ & $0.48$ & - & $40.96$ & $3.9$ & j\\
11283132$+$5833417 & $172.13052$ & $58.56161$ & $0.01022$ & $44.0$ & $8.6$ & $0.68$ & - & $39.30$ & $0.48$ & p\\
11330509$-$0400474 & $173.27127$ & $-4.01321$ & $0.05196$ & $228.4$ & $10.7$ & $1.0$ & - & $40.90$ & $9.2$ & j\\
11335920$+$4903432 & $173.49678$ & $49.06204$ & $0.03162$ & $138.1$ & $10.3$ & $0.88$ & - & $40.41$ & $2.0$ & j\\
11344658$+$4857217 & $173.69408$ & $48.95607$ & $0.03157$ & $137.8$ & $11.2$ & $0.41$ & - & $40.07$ & $4.6$ & j\\
11362642$+$7009268 & $174.11006$ & $70.15752$ & $0.04528$ & $202.4$ & $11.6$ & $0.33$ & - & $40.31$ & $0.52$ & j\\
11390851$+$5539527 & $174.78558$ & $55.66459$ & $0.06148$ & $278.7$ & $11.3$ & $0.28$ & - & $40.51$ & $1.6$ & j\\
11401689$+$1743404 & $175.07042$ & $17.72792$ & $0.01158$ & $52.0$ & $9.0$ & $1.1$ & - & $39.67$ & $0.49$ & p\\
11450498$+$1936229 & $176.27083$ & $19.60635$ & $0.02160$ & $91.2$ & $9.7$ & $5.7$ & - & $40.86$ & $6.1$ & j\\
11452010$-$3425596 & $176.33388$ & $-34.43320$ & $0.06817$ & $305.7$ & $11.1$ & $0.38$ & $0.54$ & $40.75$ & $1.2$ & j\\
11463354$-$3300247 & $176.63988$ & $-33.00685$ & $0.06024$ & $266.9$ & $11.3$ & $0.46$ & $0.62$ & $40.70$ & $1.6$ & j\\
11472209$+$3501071 & $176.84215$ & $35.01873$ & $0.06289$ & $284.0$ & $11.5$ & $0.64$ & - & $40.89$ & $0.32$ & p\\
11485036$+$5924561 & $177.20985$ & $59.41562$ & $0.01075$ & $45.8$ & $8.6$ & $0.48$ & - & $39.19$ & $0.30$ & p\\
11553166$+$5453565 & $178.88199$ & $54.89898$ & $0.05174$ & $231.8$ & $11.2$ & $1.5$ & - & $41.10$ & $1.9$ & j\\
11564844$-$0405406 & $179.20183$ & $-4.09455$ & $0.02685$ & $111.2$ & $10.4$ & $0.36$ & - & $39.83$ & $7.4$ & j\\
11590561$+$5820355 & $179.77351$ & $58.34325$ & $0.05526$ & $241.4$ & $11.5$ & $0.34$ & - & $40.48$ & $10$ & j\\
12015317$-$1852379 & $180.47154$ & $-18.87720$ & $0.00569$ & $24.4$ & $7.2$ & $0.58$ & - & $38.72$ & $1.8$ & g\\
12030709$+$5140307 & $180.77959$ & $51.67518$ & $0.06340$ & $287.8$ & $11.6$ & $0.68$ & - & $40.94$ & $3.1$ & j\\
12040140$+$2013559 & $181.00592$ & $20.23227$ & $0.02445$ & $103.9$ & $9.9$ & $0.40$ & - & $39.82$ & $6.8$ & j\\
12053418$+$5032205 & $181.39246$ & $50.53903$ & $0.00253$ & $14.9$ & $7.5$ & $0.22$ & - & $37.88$ & $3.1$ & g\\
12062311$+$5242394 & $181.59631$ & $52.71095$ & $0.00282$ & $17.2$ & $7.8$ & $0.27$ & - & $38.09$ & $0.28$ & p\\
12063333$+$2215375 & $181.63892$ & $22.26040$ & $0.06506$ & $293.6$ & $11.5$ & $0.92$ & - & $41.08$ & $0.69$ & p\\
12070524$-$2741466 & $181.77185$ & $-27.69632$ & $0.02507$ & $103.9$ & $10.1$ & $0.28$ & - & $39.67$ & $17$ & j\\
12080557$+$2514141 & $182.02316$ & $25.23728$ & $0.02253$ & $95.7$ & $10.3$ & $0.75$ & - & $40.02$ & $14$ & j\\
12103265$+$3924207 & $182.63608$ & $39.40576$ & $0.00332$ & $14.7$ & $7.5$ & $0.36$ & - & $38.08$ & $0.31$ & p\\
12110780$-$4641240 & $182.78250$ & $-46.68995$ & $0.03268$ & $137.6$ & $10.9$ & - & $0.41$ & $39.94$ & $2.0$ & j\\
12154383$+$1709178 & $183.93260$ & $17.15489$ & $0.09563$ & $449.5$ & $11.6$ & $0.49$ & - & $41.18$ & $1.1$ & j\\
12184962$+$1424593 & $184.70677$ & $14.41649$ & $0.00803$ & $33.5$ & $7.1$ & $0.42$ & - & $38.86$ & $5.2$ & g\\
12185235$+$0514443 & $184.71819$ & $5.24564$ & $0.07528$ & $343.3$ & $11.5$ & $0.50$ & - & $40.96$ & $0.33$ & p\\
12185761$+$4718133 & $184.74008$ & $47.30372$ & $0.00149$ & $7.4$ & $5.6$ & $0.51$ & - & $37.64$ & $8.1$ & g\\
12192326$+$0549289 & $184.84692$ & $5.82471$ & $0.00747$ & $32.1$ & $7.4$ & $10$ & - & $40.22$ & $5.1$ & j\\
12200682$+$2916498 & $185.02841$ & $29.28050$ & $0.00216$ & $15.1$ & $7.3$ & $0.39$ & - & $38.13$ & $0.28$ & p\\
12215494$+$0428249 & $185.47896$ & $4.47359$ & $0.00522$ & $22.1$ & $7.0$ & $0.44$ & - & $38.52$ & $2.6$ & g\\
12225489$+$1549205 & $185.72874$ & $15.82238$ & $0.00524$ & $20.3$ & $6.8$ & $0.26$ & - & $38.22$ & $6.9$ & g\\
12250377$+$1253130 & $186.26575$ & $12.88696$ & $0.00354$ & $17.3$ & $6.3$ & $6.1$ & - & $39.44$ & $2.0$ & j\\
12262708$+$3113247 & $186.61293$ & $31.22352$ & $0.00239$ & $16.8$ & $7.0$ & $0.24$ & - & $38.02$ & $1.2$ & g\\
12262960$+$0901094 & $186.62328$ & $9.01927$ & $0.02524$ & $106.7$ & $9.5$ & $0.30$ & - & $39.71$ & $4.4$ & j\\
12281111$+$4405368 & $187.04633$ & $44.09356$ & $0.00069$ & $6.5$ & $7.5$ & $0.27$ & - & $37.24$ & $6.7$ & g\\
12290674$+$0203083 & $187.27812$ & $2.05233$ & $0.15834$ & $809.6$ & $9.9$ & $55$ & - & $43.74$ & $0.36$ & j\\
12294679$+$0800014 & $187.44499$ & $8.00041$ & $0.00333$ & $15.8$ & $5.5$ & $0.26$ & - & $37.99$ & $2.6$ & j\\
12295233$+$1140391 & $187.46806$ & $11.67747$ & $0.08279$ & $382.0$ & $11.3$ & $1.6$ & - & $41.54$ & $3.1$ & j\\
12301214$+$1144411 & $187.55058$ & $11.74488$ & $0.08710$ & $404.3$ & $11.6$ & $0.38$ & - & $40.98$ & $0.30$ & p\\
12303636$+$4138370 & $187.65154$ & $41.64363$ & $0.00189$ & $10.2$ & $7.5$ & $0.81$ & - & $38.11$ & $6.5$ & g\\
12304942$+$1223279 & $187.70593$ & $12.39110$ & $0.00436$ & $18.4$ & $5.9$ & $1.5\times 10^{2}$ & - & $40.88$ & $8.8$ & j\\
12311545$-$3346248 & $187.81439$ & $-33.77355$ & $0.05629$ & $247.9$ & $11.5$ & $0.50$ & $0.60$ & $40.67$ & $1.2$ & j\\
12315921$+$1425134 & $187.99673$ & $14.42041$ & $0.00761$ & $31.6$ & $6.3$ & $0.28$ & - & $38.62$ & $2.0$ & g\\
12360813$+$1638291 & $189.03391$ & $16.64143$ & $0.07890$ & $362.6$ & $11.5$ & $0.68$ & - & $41.13$ & $1.4$ & j\\
12410031$+$1833142 & $190.25134$ & $18.55391$ & $0.07375$ & $336.7$ & $11.7$ & $0.60$ & - & $41.02$ & $2.7$ & j\\
12420800$+$3232294 & $190.53337$ & $32.54151$ & $0.00202$ & $8.5$ & $6.6$ & $0.98$ & - & $38.03$ & $9.7$ & g\\
12450867$-$0027428 & $191.28615$ & $-0.46191$ & $0.00508$ & $22.4$ & $7.1$ & $0.43$ & - & $38.52$ & $1.7$ & g\\
12484927$-$4118399 & $192.20532$ & $-41.31109$ & $0.00987$ & $41.7$ & $7.3$ & - & $5.7$ & $40.04$ & $0.0$ & p\\
12505314$+$4107125 & $192.72145$ & $41.12015$ & $0.00103$ & $5.5$ & $5.2$ & $0.27$ & - & $37.09$ & $1.7$ & g\\
12520837$-$2151544 & $193.03496$ & $-21.86511$ & $0.02318$ & $96.0$ & $9.8$ & $0.22$ & - & $39.50$ & $9.9$ & j\\
12525601$-$1520318 & $193.23346$ & $-15.34223$ & $0.04462$ & $193.6$ & $11.6$ & $0.35$ & - & $40.30$ & $3.2$ & j\\
12530723$-$1029394 & $193.28012$ & $-10.49428$ & $0.01478$ & $67.4$ & $8.7$ & $1.0$ & - & $39.85$ & $15$ & j\\
12542222$-$2900466 & $193.59261$ & $-29.01296$ & $0.05410$ & $237.7$ & $10.4$ & $0.38$ & - & $40.52$ & $2.5$ & j\\
12543570$-$1234070 & $193.64874$ & $-12.56861$ & $0.01540$ & $69.4$ & $8.2$ & $7.7$ & - & $40.75$ & $4.4$ & j\\
12543771$+$5305241 & $193.65724$ & $53.09003$ & $0.05409$ & $243.0$ & $11.0$ & $0.31$ & - & $40.44$ & $4.1$ & j\\
12545745$-$4424564 & $193.73950$ & $-44.41573$ & $0.04110$ & $176.3$ & $10.8$ & - & $0.37$ & $40.11$ & $0.0$ & j\\
12561432$+$5652244 & $194.05971$ & $56.87345$ & $0.04217$ & $187.2$ & $8.9$ & $0.31$ & - & $40.22$ & $0.31$ & j\\
12572192$-$3021485 & $194.34143$ & $-30.36356$ & $0.05425$ & $238.4$ & $10.8$ & $1.2$ & $1.8$ & $41.05$ & $0.68$ & j\\
12592333$+$2754418 & $194.84727$ & $27.91161$ & $0.02288$ & $97.7$ & $10.8$ & $0.44$ & - & $39.80$ & $4.6$ & j\\
12594900$-$2539389 & $194.95415$ & $-25.66078$ & $0.06480$ & $289.7$ & $11.7$ & $0.71$ & - & $40.96$ & $0.81$ & j\\
13010079$-$3226289 & $195.25330$ & $-32.44135$ & $0.01704$ & $73.4$ & $8.6$ & $1.4$ & $1.9$ & $40.07$ & $4.8$ & j\\
13052727$-$4928044 & $196.36366$ & $-49.46790$ & $0.00188$ & $3.9$ & $4.5$ & - & $5.9$ & $38.00$ & $2.6$ & g\\
13075472$-$3146415 & $196.97794$ & $-31.77820$ & $0.05315$ & $233.2$ & $11.5$ & $0.36$ & - & $40.47$ & $1.6$ & j\\
13112384$-$4422400 & $197.84927$ & $-44.37778$ & $0.05030$ & $219.4$ & $10.4$ & - & $1.00$ & $40.73$ & $5.1$ & j\\
13154932$+$4201454 & $198.95554$ & $42.02929$ & $0.00161$ & $10.1$ & $5.7$ & $0.36$ & - & $37.74$ & $6.8$ & g\\
13161700$+$0702465 & $199.07089$ & $7.04624$ & $0.05014$ & $221.0$ & $10.4$ & $2.0$ & - & $41.18$ & $6.7$ & j\\
13191657$-$0055009 & $199.81908$ & $-0.91702$ & $0.08186$ & $376.7$ & $11.3$ & $0.50$ & - & $41.03$ & $3.8$ & j\\
13195002$-$2724362 & $199.95851$ & $-27.41009$ & $0.00715$ & $30.1$ & $7.1$ & $0.26$ & - & $38.56$ & $0.33$ & p\\
13211286$-$4342168 & $200.30356$ & $-43.70469$ & $0.01141$ & $46.9$ & $7.6$ & - & $13$ & $40.50$ & $9.4$ & j\\
13222448$-$1643420 & $200.60196$ & $-16.72844$ & $0.01692$ & $73.8$ & $9.8$ & $0.27$ & - & $39.36$ & $0.29$ & p\\
13234497$+$3133568 & $200.93747$ & $31.56576$ & $0.01618$ & $70.7$ & $9.6$ & $2.0$ & - & $40.18$ & $12$ & j\\
13245144$+$3622424 & $201.21439$ & $36.37854$ & $0.01749$ & $77.6$ & $9.8$ & $0.88$ & - & $39.90$ & $0.54$ & j\\
13252775$-$4301073 & $201.36565$ & $-43.01871$ & $0.00182$ & $3.6$ & $3.9$ & - & $1.8\times 10^{3}$ & $40.42$ & $73$ & j\\
13261057$-$2725386 & $201.54411$ & $-27.42740$ & $0.04372$ & $189.1$ & $10.9$ & $1.6$ & - & $40.94$ & $3.6$ & j\\
13264647$-$2707078 & $201.69371$ & $-27.11891$ & $0.04352$ & $188.2$ & $11.4$ & $0.25$ & - & $40.14$ & $1.2$ & j\\
13295269$+$4711429 & $202.46957$ & $47.19526$ & $0.00154$ & $8.8$ & $5.6$ & $1.0$ & - & $38.07$ & $13$ & g\\
13322574$-$3308100 & $203.10728$ & $-33.13604$ & $0.04906$ & $213.9$ & $11.1$ & - & $2.2$ & $41.04$ & $0.96$ & u\\
13324251$+$0719382 & $203.17723$ & $7.32729$ & $0.02367$ & $98.7$ & $10.2$ & $0.30$ & - & $39.65$ & $8.1$ & j\\
13344779$-$2707374 & $203.69919$ & $-27.12709$ & $0.03481$ & $148.2$ & $10.3$ & $0.43$ & - & $40.16$ & $6.3$ & j\\
13351273$-$1122361 & $203.80302$ & $-11.37677$ & $0.07003$ & $316.5$ & $11.4$ & $0.23$ & - & $40.54$ & $2.0$ & j\\
13360823$-$0829519 & $204.03436$ & $-8.49774$ & $0.02280$ & $95.2$ & $9.3$ & $0.39$ & - & $39.73$ & $4.0$ & j\\
13363905$-$3357572 & $204.16269$ & $-33.96588$ & $0.01247$ & $51.1$ & $7.6$ & $2.4$ & $26$ & $40.89$ & $17$ & j\\
13370091$-$2951567 & $204.25383$ & $-29.86576$ & $0.00171$ & $4.8$ & $4.7$ & $1.1$ & - & $37.57$ & $8.3$ & g\\
13414914$+$2622248 & $205.45474$ & $26.37356$ & $0.07573$ & $347.7$ & $11.3$ & $0.37$ & - & $40.83$ & $2.5$ & j\\
13434918$-$1949278 & $205.95497$ & $-19.82434$ & $0.03285$ & $139.7$ & $11.0$ & $0.23$ & - & $39.84$ & $3.3$ & j\\
13444152$+$4028027 & $206.17303$ & $40.46738$ & $0.07554$ & $347.8$ & $11.6$ & $0.23$ & - & $40.62$ & $4.6$ & j\\
13462397$-$3758155 & $206.59991$ & $-37.97103$ & $0.03761$ & $160.6$ & $10.8$ & $0.88$ & $1.2$ & $40.55$ & $4.0$ & j\\
13471216$-$2422224 & $206.80067$ & $-24.37294$ & $0.01953$ & $82.0$ & $10.0$ & $0.59$ & - & $39.78$ & $6.8$ & j\\
13485251$+$2635348 & $207.21877$ & $26.59296$ & $0.06326$ & $285.8$ & $11.2$ & $0.92$ & - & $41.06$ & $0.31$ & p\\
13521776$+$3126460 & $208.07411$ & $31.44619$ & $0.04519$ & $199.7$ & $11.0$ & $4.8$ & - & $41.47$ & $2.3$ & j\\
13560288$+$1822188 & $209.01202$ & $18.37190$ & $0.05000$ & $221.4$ & $10.1$ & $0.38$ & - & $40.45$ & $0.31$ & p\\
13571620$-$2523251 & $209.31758$ & $-25.39029$ & $0.03786$ & $162.3$ & $11.0$ & $0.59$ & - & $40.37$ & $0.82$ & j\\
13595556$-$1056266 & $209.98152$ & $-10.94078$ & $0.05969$ & $266.0$ & $11.5$ & $0.29$ & - & $40.50$ & $2.9$ & j\\
14014186$-$1136251 & $210.42441$ & $-11.60697$ & $0.03669$ & $157.7$ & $10.1$ & $2.0$ & - & $40.89$ & $6.9$ & j\\
14033877$-$3358422 & $210.91154$ & $-33.97839$ & $0.01376$ & $57.4$ & $7.7$ & $0.37$ & $0.61$ & $39.35$ & $3.7$ & j\\
14070036$+$2827141 & $211.75163$ & $28.45403$ & $0.07658$ & $352.3$ & $11.6$ & $0.82$ & - & $41.19$ & $0.28$ & p\\
14071554$-$2709293 & $211.81485$ & $-27.15820$ & $0.02417$ & $100.7$ & $10.1$ & $0.27$ & - & $39.63$ & $6.6$ & j\\
14072978$-$2701043 & $211.87405$ & $-27.01787$ & $0.02180$ & $90.3$ & $9.7$ & $0.65$ & - & $39.90$ & $0.24$ & p\\
14095733$+$1732435 & $212.48880$ & $17.54548$ & $0.01619$ & $72.1$ & $9.0$ & $0.81$ & - & $39.80$ & $3.8$ & j\\
14102887$-$4246555 & $212.62038$ & $-42.78210$ & $0.05139$ & $224.9$ & $11.4$ & - & $2.5$ & $41.15$ & $1.3$ & j\\
14131490$-$0312272 & $213.31209$ & $-3.20756$ & $0.00618$ & $26.9$ & $8.2$ & $0.34$ & - & $38.57$ & $0.28$ & p\\
14165292$+$1048264 & $214.22060$ & $10.80737$ & $0.02471$ & $105.2$ & $8.9$ & $4.4$ & - & $40.87$ & $7.5$ & j\\
14200369$-$4935424 & $215.01541$ & $-49.59509$ & $0.09142$ & $424.7$ & $11.7$ & - & $4.6$ & $41.97$ & $8.7$ & p\\
14244053$+$2637303 & $216.16887$ & $26.62511$ & $0.03713$ & $162.3$ & $11.3$ & $0.86$ & - & $40.54$ & $1.8$ & j\\
14295539$+$0715129 & $217.48076$ & $7.25356$ & $0.05509$ & $245.2$ & $11.0$ & $2.1$ & - & $41.28$ & $13$ & j\\
14313860$-$4325060 & $217.91092$ & $-43.41844$ & $0.00658$ & $25.3$ & $8.6$ & - & $0.31$ & $38.35$ & $0.99$ & g\\
14401795$+$0556341 & $220.07487$ & $5.94279$ & $0.06111$ & $274.3$ & $11.6$ & $0.33$ & - & $40.58$ & $7.3$ & j\\
14413371$-$3754543 & $220.39041$ & $-37.91516$ & $0.03953$ & $169.9$ & $11.3$ & $0.49$ & $0.79$ & $40.41$ & $0.60$ & u\\
14441768$-$4357434 & $221.07378$ & $-43.96202$ & $0.07024$ & $316.7$ & $11.6$ & - & $0.36$ & $40.61$ & $2.8$ & j\\
14492161$+$6316142 & $222.33997$ & $63.27056$ & $0.04168$ & $185.7$ & $10.8$ & $3.0$ & - & $41.20$ & $0.29$ & p\\
14535765$+$0332401 & $223.49016$ & $3.54451$ & $0.00561$ & $24.8$ & $7.7$ & $0.28$ & - & $38.42$ & $3.5$ & g\\
14542347$+$1621187 & $223.59776$ & $16.35524$ & $0.04527$ & $199.6$ & $10.3$ & $1.5$ & - & $40.95$ & $5.6$ & j\\
14550964$-$3655077 & $223.79013$ & $-36.91878$ & $0.09466$ & $442.4$ & $11.5$ & $1.2$ & - & $41.55$ & $2.4$ & j\\
14555524$+$1151407 & $223.98022$ & $11.86140$ & $0.03168$ & $136.8$ & $10.3$ & $0.41$ & - & $40.07$ & $5.0$ & j\\
14592480$-$1641365 & $224.85329$ & $-16.69347$ & $0.01164$ & $46.9$ & $9.4$ & $1.2$ & - & $39.60$ & $0.31$ & p\\
15031519$+$3608520 & $225.81320$ & $36.14774$ & $0.07339$ & $337.3$ & $11.7$ & $0.40$ & - & $40.84$ & $1.1$ & j\\
15041584$+$2834110 & $226.06607$ & $28.56975$ & $0.05839$ & $262.9$ & $11.6$ & $1.8$ & - & $41.27$ & $14$ & j\\
15061668$-$4325285 & $226.56960$ & $-43.42464$ & $0.05591$ & $246.9$ & $10.8$ & - & $0.39$ & $40.42$ & $1.1$ & u\\
15064449$+$3428232 & $226.68536$ & $34.47312$ & $0.11117$ & $536.4$ & $11.7$ & $0.22$ & - & $40.99$ & $1.1$ & j\\
15072530$+$0829446 & $226.85547$ & $8.49571$ & $0.07889$ & $363.3$ & $11.5$ & $0.33$ & - & $40.82$ & $5.8$ & j\\
15104145$-$4512216 & $227.67276$ & $-45.20602$ & $0.03453$ & $147.0$ & $10.5$ & - & $0.44$ & $40.03$ & $3.2$ & j\\
15105610$+$0544416 & $227.73375$ & $5.74490$ & $0.02149$ & $91.2$ & $10.3$ & $0.53$ & - & $39.83$ & $0.91$ & j\\
15112652$+$0620568 & $227.86052$ & $6.34910$ & $0.08096$ & $373.7$ & $11.2$ & $0.57$ & - & $41.08$ & $0.44$ & j\\
15144933$+$1017035 & $228.70563$ & $10.28426$ & $0.05724$ & $256.2$ & $11.7$ & $0.44$ & - & $40.64$ & $1.2$ & j\\
15161186$-$3819218 & $229.04951$ & $-38.32278$ & $0.03914$ & $168.4$ & $10.6$ & $2.1\times 10^{-2}$ & $1.2$ & $40.57$ & $14$ & j\\
15164020$+$0015017 & $229.16756$ & $0.25052$ & $0.05259$ & $233.3$ & $11.6$ & $2.7$ & - & $41.34$ & $4.2$ & j\\
15164448$+$0701180 & $229.18536$ & $7.02164$ & $0.03446$ & $149.4$ & $9.9$ & $5.5$ & - & $41.27$ & $0.42$ & j\\
15174180$-$2422192 & $229.42424$ & $-24.37206$ & $0.04903$ & $215.0$ & $10.9$ & $2.0$ & - & $41.16$ & $0.31$ & p\\
15183652$-$2404069 & $229.65219$ & $-24.06859$ & $0.00856$ & $34.0$ & $8.2$ & $0.26$ & - & $38.66$ & $7.3$ & g\\
15212251$+$0420304 & $230.34389$ & $4.34174$ & $0.05216$ & $231.6$ & $11.3$ & $0.52$ & - & $40.63$ & $7.4$ & j\\
15305641$+$8227211 & $232.73450$ & $82.45585$ & $0.02210$ & $96.9$ & $9.6$ & $0.23$ & - & $39.51$ & $9.1$ & j\\
15345727$+$2330104 & $233.73863$ & $23.50291$ & $0.01813$ & $79.3$ & $9.9$ & $0.33$ & - & $39.49$ & $0.29$ & p\\
15385414$+$1701344 & $234.72560$ & $17.02622$ & $0.03011$ & $128.5$ & $10.8$ & $0.26$ & - & $39.82$ & $11$ & j\\
15433394$+$0452190 & $235.89139$ & $4.87199$ & $0.03996$ & $174.7$ & $10.5$ & $0.28$ & - & $40.12$ & $0.32$ & p\\
15564156$-$3302185 & $239.17329$ & $-33.03860$ & $0.06556$ & $294.6$ & $11.6$ & $1.1$ & $1.3$ & $41.15$ & $4.5$ & j\\
15572135$+$5440163 & $239.33905$ & $54.67116$ & $0.04712$ & $211.1$ & $11.1$ & $0.27$ & - & $40.27$ & $6.8$ & j\\
15573014$+$7041207 & $239.37575$ & $70.68913$ & $0.02572$ & $113.8$ & $9.8$ & $2.0$ & - & $40.59$ & $13$ & j\\
15582195$-$1409585 & $239.59146$ & $-14.16630$ & $0.09741$ & $458.9$ & $11.5$ & $0.47$ & - & $41.18$ & $0.87$ & p\\
15590169$+$5924216 & $239.75703$ & $59.40606$ & $0.06020$ & $273.9$ & $11.2$ & $0.22$ & - & $40.40$ & $1.0$ & p\\
16033205$+$1711546 & $240.88365$ & $17.19862$ & $0.03402$ & $148.5$ & $10.6$ & $0.69$ & - & $40.37$ & $5.7$ & j\\
16045670$+$2355583 & $241.23622$ & $23.93283$ & $0.03195$ & $139.6$ & $9.7$ & $0.66$ & - & $40.29$ & $1.9$ & j\\
16050900$+$1743478 & $241.28751$ & $17.72993$ & $0.03126$ & $136.1$ & $10.8$ & $0.79$ & - & $40.35$ & $0.60$ & p\\
16061598$+$1814592 & $241.56670$ & $18.24988$ & $0.03690$ & $161.8$ & $10.5$ & $0.42$ & - & $40.22$ & $11$ & j\\
16082116$+$2828436 & $242.08815$ & $28.47874$ & $0.05018$ & $224.3$ & $11.7$ & $0.24$ & - & $40.26$ & $3.7$ & j\\
16103572$-$0511173 & $242.64885$ & $-5.18808$ & $0.07300$ & $333.4$ & $11.7$ & $0.38$ & - & $40.81$ & $5.1$ & j\\
16174059$+$3500154 & $244.41904$ & $35.00427$ & $0.02981$ & $130.7$ & $10.5$ & $2.1$ & - & $40.75$ & $9.7$ & j\\
16190828$-$0304316 & $244.78461$ & $-3.07548$ & $0.06841$ & $310.7$ & $11.2$ & $0.64$ & - & $40.97$ & $1.3$ & j\\
16230308$+$3755204 & $245.76292$ & $37.92236$ & $0.03103$ & $136.4$ & $9.7$ & $0.44$ & - & $40.09$ & $0.55$ & j\\
16263817$-$3633198 & $246.65906$ & $-36.55548$ & $0.04325$ & $188.1$ & $10.9$ & $0.27$ & $0.35$ & $40.16$ & $1.3$ & j\\
16280407$+$5146311 & $247.01692$ & $51.77540$ & $0.05470$ & $247.2$ & $11.2$ & $0.67$ & - & $40.79$ & $12$ & j\\
16283827$+$3933049 & $247.15945$ & $39.55135$ & $0.03103$ & $136.6$ & $9.3$ & $3.7$ & - & $41.02$ & $1.2$ & j\\
16323175$+$8232165 & $248.13274$ & $82.53791$ & $0.02471$ & $109.7$ & $9.1$ & $2.0$ & - & $40.56$ & $6.9$ & j\\
16390277$-$6505079 & $249.76155$ & $-65.08545$ & $0.04937$ & $215.8$ & $11.1$ & - & $0.83$ & $40.64$ & $6.9$ & j\\
16393265$+$5346437 & $249.88596$ & $53.77881$ & $0.11005$ & $532.2$ & $11.7$ & $0.68$ & - & $41.47$ & $1.7$ & j\\
16441613$-$7715491 & $251.06717$ & $-77.26359$ & $0.04270$ & $184.4$ & $11.3$ & - & $8.3$ & $41.50$ & $6.5$ & j\\
16452053$-$7335141 & $251.33554$ & $-73.58723$ & $0.06942$ & $312.7$ & $11.1$ & - & $0.89$ & $40.99$ & $0.0$ & p\\
16503901$+$1200274 & $252.66261$ & $12.00770$ & $0.08456$ & $393.9$ & $11.7$ & $0.28$ & - & $40.81$ & $0.55$ & j\\
16505893$+$8134292 & $252.74521$ & $81.57473$ & $0.03791$ & $169.4$ & $11.0$ & $0.31$ & - & $40.13$ & $4.6$ & j\\
16525886$+$0224035 & $253.24535$ & $2.40102$ & $0.02448$ & $105.4$ & $9.1$ & $0.43$ & - & $39.86$ & $0.25$ & p\\
16535220$+$3945369 & $253.46756$ & $39.76019$ & $0.03366$ & $148.7$ & $9.7$ & $1.6$ & - & $40.72$ & $0.33$ & p\\
16535808$-$0510173 & $253.49203$ & $-5.17151$ & $0.07227$ & $330.3$ & $11.5$ & $0.37$ & - & $40.79$ & $3.0$ & j\\
16582659$-$6116553 & $254.61082$ & $-61.28204$ & $0.04921$ & $215.3$ & $10.9$ & - & $0.98$ & $40.71$ & $1.3$ & j\\
17004523$+$3008129 & $255.18846$ & $30.13694$ & $0.03442$ & $151.8$ & $11.2$ & $0.69$ & - & $40.38$ & $2.3$ & j\\
17050125$-$2445099 & $256.25528$ & $-24.75273$ & $0.03629$ & $157.1$ & $10.8$ & $3.3$ & - & $41.10$ & $8.9$ & j\\
17050269$+$6849389 & $256.26135$ & $68.82752$ & $0.04050$ & $181.1$ & $10.4$ & $0.25$ & - & $40.10$ & $1.8$ & j\\
17052935$+$2216075 & $256.37225$ & $22.26876$ & $0.04959$ & $221.7$ & $11.0$ & $0.42$ & - & $40.50$ & $1.5$ & j\\
17053973$-$1450498 & $256.41556$ & $-14.84714$ & $0.04250$ & $186.2$ & $11.4$ & $0.23$ & - & $40.09$ & $0.63$ & j\\
17090816$+$0923583 & $257.28412$ & $9.39945$ & $0.03599$ & $157.8$ & $10.8$ & $0.77$ & - & $40.47$ & $1.4$ & j\\
17092831$-$2226505 & $257.36795$ & $-22.44737$ & $0.03095$ & $133.0$ & $10.3$ & $0.58$ & - & $40.19$ & $16$ & j\\
17105840$+$4624210 & $257.74335$ & $46.40585$ & $0.03680$ & $163.5$ & $10.8$ & $0.46$ & - & $40.27$ & $8.5$ & j\\
17115542$-$2309423 & $257.98090$ & $-23.16181$ & $0.02685$ & $114.6$ & $10.5$ & $0.36$ & - & $39.86$ & $3.4$ & j\\
17124278$-$2435477 & $258.17828$ & $-24.59663$ & $0.02433$ & $103.3$ & $9.7$ & $1.3$ & - & $40.32$ & $8.4$ & j\\
17131541$-$2502266 & $258.31430$ & $-25.04076$ & $0.02857$ & $122.2$ & $10.0$ & $7.2$ & - & $41.21$ & $3.0$ & j\\
17154136$-$1206217 & $258.92233$ & $-12.10608$ & $0.05790$ & $259.4$ & $11.2$ & $0.98$ & - & $41.00$ & $4.3$ & j\\
17202814$-$0058471 & $260.11731$ & $-0.97968$ & $0.03042$ & $132.1$ & $10.8$ & $56$ & - & $42.17$ & $3.1$ & j\\
17204089$-$0111573 & $260.17044$ & $-1.19920$ & $0.02860$ & $123.9$ & $10.6$ & $0.76$ & - & $40.25$ & $2.2$ & u\\
17234103$-$6500371 & $260.92096$ & $-65.01024$ & $0.01443$ & $59.0$ & $9.3$ & - & $3.7$ & $40.16$ & $0.0$ & p\\
17243782$-$0243062 & $261.15756$ & $-2.71830$ & $0.03323$ & $144.7$ & $10.3$ & $2.4$ & - & $40.89$ & $1.4$ & u\\
17323302$+$7124105 & $263.13766$ & $71.40287$ & $0.05900$ & $268.9$ & $11.6$ & $0.61$ & - & $40.82$ & $3.0$ & j\\
17331261$+$7046295 & $263.30234$ & $70.77493$ & $0.04080$ & $182.7$ & $11.4$ & $0.24$ & - & $40.08$ & $3.9$ & j\\
17354374$-$0720527 & $263.93222$ & $-7.34798$ & $0.02426$ & $104.3$ & $9.5$ & $0.57$ & - & $39.98$ & $0.72$ & j\\
17383577$+$3256010 & $264.64905$ & $32.93370$ & $0.07332$ & $338.4$ & $11.4$ & $0.25$ & - & $40.63$ & $0.45$ & j\\
17413827$+$1720172 & $265.40945$ & $17.33816$ & $0.06000$ & $271.8$ & $11.7$ & $1.6$ & - & $41.25$ & $1.3$ & j\\
17425069$+$1612507 & $265.71130$ & $16.21402$ & $0.03179$ & $139.5$ & $10.6$ & $0.66$ & - & $40.29$ & $0.32$ & p\\
17435781$+$1935091 & $265.99097$ & $19.58592$ & $0.08400$ & $392.1$ & $11.7$ & $0.57$ & - & $41.12$ & $3.8$ & j\\
17445666$+$5542166 & $266.23596$ & $55.70470$ & $0.03042$ & $135.1$ & $10.1$ & $0.80$ & - & $40.34$ & $5.9$ & j\\
17480808$+$5123570 & $267.03369$ & $51.39918$ & $0.02266$ & $100.3$ & $10.8$ & $0.56$ & - & $39.93$ & $1.7$ & j\\
17554844$+$6236435 & $268.95184$ & $62.61216$ & $0.02746$ & $122.0$ & $9.7$ & $0.30$ & - & $39.83$ & $1.1$ & p\\
18065063$+$6949275 & $271.71109$ & $69.82441$ & $0.05100$ & $230.6$ & $10.9$ & $2.1$ & - & $41.23$ & $4.8$ & j\\
18071483$-$7012383 & $271.81192$ & $-70.21067$ & $0.04006$ & $172.7$ & $10.9$ & - & $1.3$ & $40.63$ & $0.0$ & p\\
18082315$+$0841030 & $272.09650$ & $8.68418$ & $0.04871$ & $217.5$ & $11.5$ & $0.24$ & - & $40.24$ & $7.5$ & j\\
18105480$+$5000459 & $272.72839$ & $50.01276$ & $0.05009$ & $226.0$ & $11.5$ & $0.48$ & - & $40.58$ & $3.1$ & j\\
18120123$+$2127486 & $273.00513$ & $21.46349$ & $0.01734$ & $72.3$ & $9.8$ & $0.34$ & - & $39.44$ & $11$ & j\\
18175610$+$3348594 & $274.48373$ & $33.81655$ & $0.07351$ & $339.8$ & $11.5$ & $0.36$ & - & $40.81$ & $2.0$ & u\\
18185802$-$5508155 & $274.74173$ & $-55.13762$ & $0.07263$ & $330.0$ & $11.5$ & - & $0.63$ & $40.88$ & $0.80$ & j\\
18212466$-$7634598 & $275.35278$ & $-76.58333$ & $0.01836$ & $73.6$ & $9.3$ & - & $0.70$ & $39.63$ & $0.0$ & p\\
18254934$+$4654088 & $276.45557$ & $46.90252$ & $0.01550$ & $64.4$ & $11.4$ & $0.37$ & - & $39.37$ & $1.4$ & u\\
18285693$+$3220047 & $277.23724$ & $32.33456$ & $0.06501$ & $297.6$ & $11.7$ & $0.35$ & - & $40.68$ & $7.0$ & j\\
18324117$-$3411274 & $278.17145$ & $-34.19094$ & $0.01856$ & $76.6$ & $9.4$ & $0.23$ & $0.32$ & $39.32$ & $0.26$ & j\\
18350342$+$3241471 & $278.76419$ & $32.69636$ & $0.05787$ & $262.8$ & $10.4$ & $5.6$ & - & $41.77$ & $2.2$ & j\\
18363966$+$1943454 & $279.16528$ & $19.72928$ & $0.01614$ & $66.8$ & $9.1$ & $1.6$ & - & $40.02$ & $12$ & j\\
18382625$+$1711496 & $279.60938$ & $17.19715$ & $0.01689$ & $69.5$ & $9.7$ & $7.3$ & - & $40.73$ & $3.4$ & j\\
18403862$-$7709285 & $280.16086$ & $-77.15794$ & $0.01817$ & $73.1$ & $9.5$ & - & $1.2$ & $39.84$ & $0.0$ & p\\
18405544$-$7555373 & $280.23105$ & $-75.92705$ & $0.04164$ & $179.9$ & $10.6$ & - & $0.85$ & $40.49$ & $0.66$ & j\\
18420899$+$7946170 & $280.53748$ & $79.77142$ & $0.05610$ & $255.1$ & $11.5$ & $12$ & - & $42.06$ & $2.8$ & j\\
18440241$+$4533298 & $281.01001$ & $45.55825$ & $0.09170$ & $434.0$ & $11.7$ & $5.6$ & - & $42.21$ & $0.58$ & p\\
18473481$+$7044010 & $281.89502$ & $70.73358$ & $0.04374$ & $196.6$ & $10.9$ & $0.26$ & - & $40.18$ & $4.2$ & j\\
18562225$-$7932421 & $284.09271$ & $-79.54500$ & $0.07078$ & $319.8$ & $11.0$ & - & $0.75$ & $40.93$ & $0.86$ & j\\
18573750$+$3800322 & $284.40628$ & $38.00895$ & $0.05521$ & $250.4$ & $10.4$ & $0.30$ & - & $40.46$ & $0.30$ & p\\
19131601$+$4706494 & $288.31668$ & $47.11375$ & $0.05484$ & $249.0$ & $11.4$ & $0.36$ & - & $40.53$ & $5.5$ & j\\
19133446$+$4201330 & $288.39362$ & $42.02578$ & $0.05443$ & $246.9$ & $11.0$ & $0.79$ & - & $40.87$ & $3.6$ & j\\
19145766$-$2552012 & $288.74026$ & $-25.86705$ & $0.06285$ & $283.9$ & $11.1$ & $0.98$ & - & $41.08$ & $6.3$ & j\\
19204300$-$3831059 & $290.17920$ & $-38.51834$ & $0.04519$ & $198.7$ & $11.5$ & $0.24$ & - & $40.16$ & $1.6$ & p\\
19260570$-$5740166 & $291.52386$ & $-57.67130$ & $0.06097$ & $272.6$ & $11.7$ & - & $1.6$ & $41.13$ & $2.8$ & j\\
19264081$+$4123284 & $291.66998$ & $41.39114$ & $0.06850$ & $315.6$ & $11.7$ & $0.22$ & - & $40.52$ & $2.5$ & j\\
19281700$-$2931442 & $292.07086$ & $-29.52901$ & $0.02442$ & $104.8$ & $9.7$ & $2.1$ & - & $40.55$ & $2.7$ & j\\
19300192$-$1509191 & $292.50800$ & $-15.15535$ & $0.08203$ & $380.9$ & $11.5$ & $1.5$ & - & $41.52$ & $2.9$ & j\\
19332496$-$3940214 & $293.35413$ & $-39.67254$ & $0.07507$ & $343.7$ & $11.2$ & $2.5$ & $3.8$ & $41.70$ & $3.3$ & j\\
19391958$-$3540497 & $294.83157$ & $-35.68044$ & $0.08769$ & $408.7$ & $11.5$ & $0.36$ & $0.52$ & $40.99$ & $0.25$ & p\\
19403422$+$7647464 & $295.14255$ & $76.79633$ & $0.05304$ & $240.6$ & $11.7$ & $0.60$ & - & $40.72$ & $8.5$ & u\\
19414211$+$5037571 & $295.42551$ & $50.63249$ & $0.02372$ & $105.7$ & $9.4$ & $3.1$ & - & $40.72$ & $5.1$ & j\\
19452422$-$5520488 & $296.35095$ & $-55.34690$ & $0.01515$ & $59.5$ & $9.1$ & - & $0.60$ & $39.37$ & $0.0$ & p\\
19521582$+$0230243 & $298.06586$ & $2.50677$ & $0.05900$ & $267.4$ & $11.4$ & $6.0$ & - & $41.82$ & $2.8$ & j\\
19592833$+$4044022 & $299.86807$ & $40.73394$ & $0.05608$ & $255.1$ & $10.4$ & $1.6\times 10^{3}$ & - & $44.20$ & $1.0$ & j\\
19595975$+$6508547 & $299.99924$ & $65.14852$ & $0.04700$ & $212.2$ & $11.5$ & $0.25$ & - & $40.23$ & $0.32$ & p\\
20161460$-$3041314 & $304.06082$ & $-30.69212$ & $0.08825$ & $412.3$ & $11.4$ & $0.85$ & $1.3$ & $41.41$ & $5.0$ & j\\
20184779$-$5242334 & $304.69922$ & $-52.70930$ & $0.05067$ & $223.8$ & $11.4$ & - & $0.31$ & $40.24$ & $1.1$ & j\\
20202637$-$0044287 & $305.10980$ & $-0.74128$ & $0.05891$ & $267.1$ & $11.7$ & $0.42$ & - & $40.66$ & $0.52$ & p\\
20225911$-$2056561 & $305.74631$ & $-20.94892$ & $0.05400$ & $242.0$ & $11.1$ & $0.43$ & - & $40.58$ & $1.3$ & j\\
20345233$+$6009132 & $308.71805$ & $60.15368$ & $0.00013$ & $5.9$ & $5.4$ & $1.4$ & - & $37.87$ & $6.4$ & g\\
20430830$-$5059054 & $310.78461$ & $-50.98485$ & $0.06543$ & $295.3$ & $11.5$ & - & $0.34$ & $40.52$ & $1.4$ & j\\
20434570$-$2633011 & $310.94046$ & $-26.55027$ & $0.04077$ & $179.5$ & $10.5$ & $2.6$ & - & $41.11$ & $4.4$ & j\\
20455226$-$5106267 & $311.46771$ & $-51.10747$ & $0.04850$ & $213.8$ & $10.4$ & - & $0.62$ & $40.50$ & $3.7$ & j\\
20470782$+$5735369 & $311.78256$ & $57.59362$ & $0.03818$ & $171.3$ & $10.3$ & $0.67$ & - & $40.47$ & $0.75$ & j\\
20490663$-$3923195 & $312.27762$ & $-39.38873$ & $0.04071$ & $178.3$ & $10.7$ & $0.35$ & $0.50$ & $40.25$ & $1.3$ & j\\
20520232$-$5704076 & $313.00974$ & $-57.06877$ & $0.01175$ & $46.6$ & $8.8$ & - & $2.2$ & $39.72$ & $1.7$ & p\\
20520957$-$5247457 & $313.03989$ & $-52.79598$ & $0.04636$ & $203.6$ & $10.9$ & - & $0.47$ & $40.34$ & $1.6$ & j\\
20530614$-$1620078 & $313.27557$ & $-16.33549$ & $0.04270$ & $189.3$ & $10.9$ & $0.38$ & - & $40.32$ & $6.3$ & j\\
20583752$-$5756359 & $314.65656$ & $-57.94333$ & $0.05242$ & $231.9$ & $11.5$ & - & $0.88$ & $40.73$ & $0.98$ & j\\
21013771$-$2801543 & $315.40710$ & $-28.03176$ & $0.03944$ & $173.4$ & $10.8$ & $5.8$ & - & $41.43$ & $12$ & j\\
21014441$-$1318475 & $315.43503$ & $-13.31322$ & $0.02943$ & $128.9$ & $10.6$ & $1.3$ & - & $40.53$ & $4.3$ & j\\
21030023$-$3058431 & $315.75107$ & $-30.97865$ & $0.03896$ & $170.9$ & $10.6$ & $0.47$ & $0.61$ & $40.32$ & $3.3$ & j\\
21072021$-$2529150 & $316.83420$ & $-25.48756$ & $0.03468$ & $151.8$ & $10.5$ & $5.0$ & - & $41.24$ & $5.3$ & j\\
21072565$-$2525430 & $316.85687$ & $-25.42866$ & $0.03842$ & $168.9$ & $10.2$ & $5.8$ & - & $41.40$ & $2.7$ & j\\
21140128$+$8204483 & $318.50482$ & $82.08009$ & $0.08400$ & $394.3$ & $11.6$ & $0.47$ & - & $41.05$ & $3.7$ & j\\
21181913$+$6048075 & $319.57962$ & $60.80207$ & $0.05555$ & $253.1$ & $11.5$ & $7.8$ & - & $41.88$ & $1.2$ & j\\
21202854$+$0246340 & $320.11887$ & $2.77621$ & $0.04700$ & $210.8$ & $11.1$ & $0.32$ & - & $40.33$ & $5.2$ & j\\
21212224$-$4635542 & $320.34265$ & $-46.59835$ & $0.07590$ & $348.0$ & $11.2$ & - & $0.35$ & $40.68$ & $0.0$ & p\\
21285092$+$0115300 & $322.21228$ & $1.25832$ & $0.04961$ & $223.1$ & $11.2$ & $0.45$ & - & $40.53$ & $2.6$ & j\\
21293744$-$2111443 & $322.40601$ & $-21.19565$ & $0.03521$ & $154.7$ & $9.9$ & $0.39$ & - & $40.15$ & $9.0$ & j\\
21313299$-$3837046 & $322.88742$ & $-38.61790$ & $0.01817$ & $75.0$ & $9.7$ & $0.98$ & $1.1$ & $39.92$ & $2.6$ & j\\
21341775$-$5338101 & $323.57385$ & $-53.63624$ & $0.07652$ & $350.6$ & $11.3$ & - & $1.2$ & $41.21$ & $1.7$ & u\\
21360902$-$6040550 & $324.03763$ & $-60.68198$ & $0.06111$ & $273.6$ & $11.5$ & - & $0.63$ & $40.72$ & $0.66$ & j\\
21410389$-$1641382 & $325.26620$ & $-16.69392$ & $0.05173$ & $232.0$ & $10.7$ & $0.25$ & - & $40.30$ & $5.6$ & j\\
21451552$-$1959406 & $326.31461$ & $-19.99468$ & $0.05870$ & $265.1$ & $11.4$ & $0.40$ & - & $40.63$ & $5.0$ & j\\
21462626$+$3332411 & $326.60934$ & $33.54472$ & $0.08720$ & $411.3$ & $11.5$ & $0.59$ & - & $41.18$ & $7.1$ & j\\
21492796$-$6429194 & $327.36664$ & $-64.48872$ & $0.05544$ & $246.0$ & $11.5$ & - & $0.94$ & $40.81$ & $1.6$ & j\\
21512991$-$5520124 & $327.87466$ & $-55.33686$ & $0.03878$ & $168.5$ & $10.8$ & - & $2.4$ & $40.88$ & $5.4$ & j\\
21515500$-$1537358 & $327.97922$ & $-15.62664$ & $0.06120$ & $277.6$ & $11.6$ & $0.57$ & - & $40.83$ & $5.7$ & j\\
21570170$-$0750224 & $329.25714$ & $-7.83958$ & $0.06203$ & $282.3$ & $11.5$ & $0.43$ & - & $40.72$ & $1.1$ & j\\
21570253$+$6626098 & $329.26047$ & $66.43603$ & $0.05843$ & $267.0$ & $10.3$ & $1.0$ & - & $41.04$ & $1.4$ & j\\
21570595$-$6941236 & $329.27487$ & $-69.68994$ & $0.02827$ & $119.8$ & $10.3$ & - & $44$ & $41.85$ & $5.6$ & j\\
22002408$-$5610413 & $330.10043$ & $-56.17819$ & $0.07578$ & $346.7$ & $11.3$ & - & $0.96$ & $41.11$ & $2.1$ & j\\
22011708$-$3746241 & $330.32111$ & $-37.77333$ & $0.03344$ & $145.4$ & $11.0$ & $1.6$ & $2.8$ & $40.82$ & $9.1$ & j\\
22041766$+$0440021 & $331.07358$ & $4.66722$ & $0.02700$ & $119.4$ & $11.2$ & $0.78$ & - & $40.23$ & $2.7$ & j\\
22111201$+$3855384 & $332.80008$ & $38.92728$ & $0.02018$ & $89.1$ & $9.7$ & $0.33$ & - & $39.60$ & $10$ & j\\
22122068$-$2518283 & $333.08624$ & $-25.30791$ & $0.06256$ & $283.6$ & $11.0$ & $0.31$ & - & $40.58$ & $1.3$ & j\\
22144500$+$1350476 & $333.68747$ & $13.84653$ & $0.02616$ & $116.2$ & $10.3$ & $3.3$ & - & $40.83$ & $6.1$ & j\\
22234962$-$0206137 & $335.95673$ & $-2.10381$ & $0.05588$ & $252.9$ & $11.1$ & $5.8$ & - & $41.75$ & $8.2$ & j\\
22275446$-$3034321 & $336.97696$ & $-30.57555$ & $0.05806$ & $261.3$ & $11.0$ & $0.89$ & $1.5$ & $41.05$ & $1.2$ & j\\
22312062$+$3921298 & $337.83585$ & $39.35825$ & $0.01713$ & $73.7$ & $9.9$ & $2.9$ & - & $40.38$ & $17$ & j\\
22314322$-$0824318 & $337.93002$ & $-8.40885$ & $0.08289$ & $386.9$ & $11.2$ & $0.76$ & - & $41.24$ & $4.3$ & j\\
22351101$-$5223239 & $338.79596$ & $-52.39006$ & $0.05501$ & $244.9$ & $11.6$ & - & $0.64$ & $40.64$ & $0.0$ & p\\
22370410$+$3424573 & $339.26709$ & $34.41592$ & $0.00272$ & $14.1$ & $6.1$ & $0.33$ & - & $37.99$ & $3.2$ & g\\
22380121$+$4107363 & $339.50519$ & $41.12675$ & $0.05742$ & $262.2$ & $11.6$ & $0.69$ & - & $40.86$ & $4.8$ & j\\
22381350$-$0702052 & $339.55634$ & $-7.03477$ & $0.00965$ & $38.8$ & $11.5$ & $0.23$ & - & $38.72$ & $1.6$ & u\\
22382946$+$3519400 & $339.62277$ & $35.32798$ & $0.02759$ & $123.4$ & $9.7$ & $0.36$ & - & $39.92$ & $0.52$ & j\\
22391136$-$1720284 & $339.79739$ & $-17.34119$ & $0.07437$ & $342.8$ & $11.6$ & $1.9$ & - & $41.53$ & $2.3$ & j\\
22423823$-$4254324 & $340.65927$ & $-42.90901$ & $0.03156$ & $136.5$ & $10.6$ & - & $0.30$ & $39.80$ & $2.5$ & j\\
22425137$-$1657082 & $340.71399$ & $-16.95232$ & $0.06716$ & $306.9$ & $11.1$ & $0.25$ & - & $40.56$ & $1.5$ & j\\
22455898$-$1737320 & $341.49582$ & $-17.62566$ & $0.06840$ & $313.0$ & $11.4$ & $0.40$ & - & $40.77$ & $0.32$ & p\\
22492263$-$3728185 & $342.34439$ & $-37.47178$ & $0.02867$ & $124.0$ & $10.1$ & $0.34$ & $0.47$ & $39.91$ & $0.97$ & j\\
22512450$+$3813414 & $342.85205$ & $38.22811$ & $0.05870$ & $268.3$ & $11.6$ & $0.99$ & - & $41.03$ & $2.3$ & j\\
22515859$+$1718147 & $342.99420$ & $17.30405$ & $0.08508$ & $399.8$ & $11.3$ & $0.71$ & - & $41.24$ & $2.7$ & j\\
22571068$-$3627449 & $344.29453$ & $-36.46248$ & $0.00571$ & $24.2$ & $6.9$ & $1.3$ & $1.1$ & $39.06$ & $2.0$ & j\\
23085823$+$2322004 & $347.24271$ & $23.36684$ & $0.03513$ & $157.1$ & $10.9$ & $0.41$ & - & $40.18$ & $1.5$ & j\\
23104223$+$0734033 & $347.67603$ & $7.56763$ & $0.04424$ & $198.4$ & $10.2$ & $1.7$ & - & $41.02$ & $5.4$ & j\\
23135863$-$4243393 & $348.49432$ & $-42.72756$ & $0.05640$ & $252.3$ & $11.2$ & - & $0.47$ & $40.53$ & $0.0$ & p\\
23161076$-$4235053 & $349.04486$ & $-42.58483$ & $0.00534$ & $21.4$ & $7.6$ & - & $0.37$ & $38.28$ & $0.0$ & p\\
23174961$+$3423504 & $349.45679$ & $34.39742$ & $0.05964$ & $272.8$ & $10.9$ & $0.40$ & - & $40.65$ & $1.3$ & j\\
23175633$-$4213335 & $349.48486$ & $-42.22595$ & $0.05600$ & $250.4$ & $11.4$ & - & $0.52$ & $40.57$ & $4.4$ & j\\
23182362$-$4222140 & $349.59842$ & $-42.37057$ & $0.00525$ & $21.8$ & $7.4$ & - & $0.40$ & $38.33$ & $0.0$ & g\\
23190591$-$4206486 & $349.77460$ & $-42.11348$ & $0.05432$ & $242.4$ & $10.8$ & - & $1.7$ & $41.06$ & $4.4$ & j\\
23204252$+$0813014 & $350.17722$ & $8.21700$ & $0.01136$ & $47.8$ & $8.1$ & $0.84$ & - & $39.47$ & $11$ & j\\
23232031$+$2035237 & $350.83472$ & $20.58990$ & $0.03802$ & $170.2$ & $10.5$ & $0.84$ & - & $40.57$ & $6.3$ & j\\
23272195$+$1524375 & $351.84149$ & $15.41040$ & $0.04597$ & $206.9$ & $11.1$ & $0.23$ & - & $40.17$ & $4.5$ & j\\
23275670$+$0846443 & $351.98627$ & $8.77900$ & $0.02892$ & $128.3$ & $10.0$ & $0.22$ & - & $39.74$ & $0.32$ & p\\
23360718$-$3230326 & $354.03000$ & $-32.50900$ & $0.05212$ & $232.7$ & $11.4$ & $0.33$ & $0.42$ & $40.44$ & $4.1$ & j\\
23382938$+$2701526 & $354.62241$ & $27.03137$ & $0.03053$ & $136.3$ & $9.4$ & $8.0$ & - & $41.36$ & $11$ & j\\
23400080$+$2708014 & $355.00342$ & $27.13372$ & $0.03135$ & $140.0$ & $9.5$ & $0.52$ & - & $40.19$ & $5.3$ & j\\
23412980$-$2919149 & $355.37415$ & $-29.32081$ & $0.05227$ & $233.6$ & $10.6$ & $0.35$ & - & $40.47$ & $6.5$ & j\\
23470479$+$5142179 & $356.77008$ & $51.70497$ & $0.04400$ & $198.5$ & $11.0$ & $0.41$ & - & $40.39$ & $2.7$ & j\\
23554421$+$3012439 & $358.93427$ & $30.21226$ & $0.03082$ & $137.7$ & $11.2$ & $0.24$ & - & $39.85$ & $0.31$ & p\\
23570068$-$3445331 & $359.25293$ & $-34.75919$ & $0.04944$ & $219.7$ & $10.0$ & $1.3$ & $3.0$ & $41.21$ & $1.0$ & j\\
23572798$+$4752129 & $359.36646$ & $47.87019$ & $0.04522$ & $204.2$ & $11.2$ & $0.67$ & - & $40.63$ & $7.3$ & j\\
23572993$+$4726219 & $359.37482$ & $47.43937$ & $0.04484$ & $202.4$ & $10.6$ & $1.8$ & - & $41.06$ & $2.1$ & j\\
23595879$+$0042066 & $359.99500$ & $0.70179$ & $0.08165$ & $381.0$ & $11.5$ & $0.44$ & - & $40.99$ & $3.8$ & j\\

